PrivacyGo: Privacy-Preserving Ad Measurement with Multidimensional Intersection

This paper tackles the challenging and practical problem of multi-identifier private user profile matching for privacy-preserving ad measurement, a cornerstone of modern advertising analytics. We introduce a comprehensive cryptographic framework leveraging reversed Oblivious Pseudorandom Functions (OPRF) and novel blind key rotation techniques to support secure matching across multiple identifiers. Our design prevents cross-identifier linkages and includes a differentially private mechanism to obfuscate intersection sizes, mitigating risks such as membership inference attacks. We present a concrete construction of our protocol that achieves both strong privacy guarantees and high efficiency. It scales to large datasets, offering a practical and scalable solution for privacy-centric applications like secure ad conversion tracking. By combining rigorous cryptographic principles with differential privacy, our work addresses a critical need in the advertising industry, setting a new standard for privacy-preserving ad measurement frameworks.

==> protocols/dp_psi_protocol.tex <==
\fbox{
    \begin{minipage}{0.45\textwidth}
    
    % \smallskip
    % \textbf{DP Budget for PSI:} 
    % \begin{itemize}
    %     \item total budget $\epsilon$, $\epsilon_1$ for cardinality protection and $\epsilon_2$ for PSI protection.
    % \end{itemize}
    
    \smallskip
    % \textbf{Inputs:} 
    \begin{itemize}
        \item Set $\eA$ according to the requirement for privacy protection of $A$.
        \item Set the subsampling rate  $p_2=\frac{e^{\eA}}{1+e^{\eA}}$ (\eg, $\eA=3$ and $p_2=0.9526$) and the upsampling parameter $q = \frac{1}{1+e^{\eA}}$.
        
        \item Set $p_1$ according to Table III-IV $\dB=\frac{1}{10n}$. 
        
        % \item The total budget is $(\epsilon, \delta)$ with $\epsilon= \epsilon_1 + \epsilon_2$ and $\delta=\delta_1=\frac{1}{10n}$.
    \end{itemize}
    
    \smallskip
 
    
    \end{minipage}
    }








==> protocols/dp_psi_stat_protocol.tex <==
\fbox{
    \begin{minipage}{0.95\textwidth}
    
    \smallskip
    \textbf{DP Budget for PSI-Stat:} 
    \begin{itemize}
        \item total budget $\epsilon$, $\epsilon_1$ for cardinality protection,  $\epsilon_2$ for PSI protection and $\epsilon_3$ for PSI-Statistics protection. 
    \end{itemize}
    
    \smallskip
    \textbf{Inputs:} 
    \begin{itemize}
        \item Set $\epsilon_2$ that meet the subsampling rate  $p_\mathsf{sub}^\mathsf{Keep}=\frac{e^{\epsilon_2}}{1+e^{\epsilon_2}}$ (\eg, $\epsilon_2=3$ and $p_\mathsf{sub}^\mathsf{Keep}=0.9526$)
        
        \item Compute $\epsilon_1$ according to (\ref{epsilon1}) by setting $\delta_1=\frac{1}{20n}$. 
        \item Compute $\epsilon^{\prime}_3$ according to (\ref{epsilon3}) by setting $\epsilon_3=3$
        \item 
        Set $\delta_3=\frac{1}{20n}$ and compute $\delta_3^{\prime}$ according to (\ref{delta3})
        \item Compute the noise variance according to (\ref{profile})
        \item The total budget is $(\epsilon, \delta)$ with $\epsilon= \epsilon_1 + \epsilon_2 + \epsilon_3$ and $\delta =\delta_1+\delta_3=\frac{1}{10n}$
    \end{itemize}
    
    \smallskip
 
    
    \end{minipage}
    }

==> protocols/dp_shuffle_protocol.tex <==
\fbox{
    \begin{minipage}{0.95\textwidth}
    
    \smallskip
    \textbf{Global Parameters:} 
    \begin{itemize}
        \item Security parameter $\lambda\in\NN^*$, Diffie-Hellman group $(1^\lambda, \GG, p, g)$, a hash function $\hash: \bin^*\to\GG$, DP parameter $\epsilon$.
    \end{itemize}
    
    \smallskip
    \textbf{Inputs:} 
    \begin{itemize}
        \item Alice: $\mathcal A = \left[a_1,\ldots, a_n\right]\in\bin^{*\times n}$.
        \item Bob: $\mathcal B = \left[b_1,\ldots, b_n\right]\in\bin^{*\times n}$,  $\mathcal{X}=\{x_{f,1},\ldots, x_{f,n}\}_{f=1}^F$.
    \end{itemize}
    
    \smallskip
    \textbf{Protocol:}
    \begin{enumerate}
        \item  Alice and Bob samples uniformly random private secret $\alpha\sample\ZZ_p$ and $\beta\sample\ZZ_p$, respectively.
        % 
        \item  Alice encrypts  $\mathcal A$ by $E_{a} = \left[\hash(a_1)^\alpha,\ldots \hash(a_n)^\alpha\right]$  and sends $E_{a}$ to Bob.
        % 
        \item 
        \begin{itemize}
            \item 
        Bob \textbf{permutes}  the order of elements in $E_a$ with random permutations $\pi$, \ie, $E^\prime_{a} \triangleq \left[\hash(a_{\pi(1)})^{\alpha },\ldots \hash(a_{\pi(n)})^{\alpha }\right]$.
% 
Then Bob encrypts $E^\prime_{a}$ to obtain $E^\prime_{a,b} \triangleq (E^\prime_{a})^{\beta} =  \left[\hash(a_{\pi_a(1)})^{\alpha \beta},\ldots \hash(a_{\pi_a(n)})^{\alpha \beta}\right]$ and sends $E^\prime_{a,b}$ back to Alice.
        
\item  Bob {\textbf {sub-samples}}  a subset $\mathcal B^\mathsf{keep}$ from  $\mathcal B$ by $\mathcal B^\mathsf{keep} = \textrm{ S}_{\text{sub}}(\mathcal B; p^\mathsf{keep}_\mathsf{sub})$ and keeps the index of the subsampled elements, \ie, $\mathsf{Idx}(\mathcal{B}^\mathsf{keep}, \mathcal B)$.  Then he encrypts  $\mathcal {B}^{\mathsf{keep}}$ by $E_b^\mathsf{keep} = [\ldots, \hash(b_i)^\beta, \ldots] $ with $b_i\in \mathcal {B}^\mathsf{keep}$. Finally, Bob sends $E_b^\mathsf{keep}$ to  Alice.
 \end{itemize}    

  \item      
        \begin{itemize}
        \item Alice  encrypts $E_{b,a}^\mathsf{keep}\triangleq(E_{b}^\mathsf{keep})^\alpha$. Then she  computes  $\widetilde {\mathcal I}_{a,b}\triangleq E_{b,a}^\mathsf{keep}\cap E^\prime_{a,b}$ and $D\triangleq E^\mathsf{keep}_{b,a}\setminus \widetilde {\mathcal I}_{a,b}$, separately. 
        \item
        Alice 
        conducts \textbf{up-sampling} by computing $ \textrm{S}_{\text{up}}(D; p^\mathsf{keep}_\mathsf{up})\cup \widetilde {\mathcal I}_{a,b}$ and sends to Bob the corresponding elements' indices in 
             $E^\mathsf{keep}_{b,a}$, \ie,  $\mathsf{Idx}(\textrm{S}_{\text{up}}(D; p^\mathsf{keep}_\mathsf{up})\cup \widetilde {\mathcal I}_{a,b}, E^\mathsf{keep}_{b,a})$.
        \end{itemize}

        \item Bob obtain $\mathcal{I}_{\text{DP}}$ by taking elements from $\mathcal B$ with   indices $\mathsf{Idx}(\textrm{S}_{\text{up}}(D; p^\mathsf{keep}_\mathsf{up})\cup \widetilde {\mathcal I}_{a,b}, E^\mathsf{keep}_{b,a})$.
        
        Bob computes DP protected statistics  $\mathcal M \left(h(\{x_{f,i}\}_{f=1}^F)\right), i\in\mathsf{Idx}(\mathcal{I}_\textrm{DP}, \mathcal{B})$ if required.
    \end{enumerate}
    
    \end{minipage}
    }

==> protocols/main_protocol.tex <==
\fbox{
    \begin{minipage}
    {0.8\textwidth} 
    
    \smallskip
    \textbf{Global Parameters:} 
    \begin{itemize} 
        \item Computational security parameter $\lambda\in\NN^*$, Diffie-Hellman group $(1^\lambda, \GG, p, g)$, and a random oracle $\hash: \bin^*\to\GG$.
        \item DP budget: $(\epsilon, \delta)$
    \end{itemize}
    
    \smallskip
    \textbf{Inputs:} 
    \begin{itemize}
        \item 
        % Each of the $m$ users in Party A has $L$ different types of PIIs. 
        The PII records at A are denoted by
 $ \mathsf{PII_A} = \left[\mathbf{a}_1,\ldots, \mathbf{a}_L\right]$ with $\mathbf{a}_{\ell}\in\bin^{*\times m}$ and $\ell\in [L]$.
 The $i$-th row and $\ell$-th column, \ie,
 $\mathbf{a}_{\ell}[i]$
 represents $i$-th user's $\ell$-th PII. %{\color{blue} and a set of values associated with each user $(v^A_1, \ldots, v^A_m)$}. 
        \item  The PII records at B follow the same ID order in A. The PII records in B are denoted by
 $\mathsf{PII_B} = \left[\mathbf{b}_1,\ldots, \mathbf{b}_L\right]$, where each $\mathbf{b}_{\ell}\in\bin^{*\times n}$. The $\ell$-th PII of the user  in the $j$-th row is denoted by $\mathbf{b}_{\ell}[j]$. %{\color{blue} and a set of values associated with each user $(v^B_1, \ldots, v^B_n)$}.
    \end{itemize}
    \smallskip
    
    \textbf{Output:}  
    \begin{itemize}
    \item $\mathsf{PII}_{\cap,A}$ at A and $\mathsf{PII}_{\cap,B}$ at B such that there exists $\ell\in [L]$ for each row $k$ in  $\mathsf{PII}_{\cap,A}$ and $\mathsf{PII}_{\cap,B}$ with $\mathbf{a}_{\ell}[j]=\mathbf{b}_{\ell}[j]$
    
    \end{itemize}
    \smallskip
    \textbf{Setup:} 
    \begin{itemize}
        \item  A and  B uniformly sample their random secrets $ \alpha_{\ell}\sample\ZZ_p$  and $\beta_{\ell}\sample\ZZ_p$ for $\ell\in [L]$. %{\color{blue} and their key pairs $(\pk_A, \sk_A), (\pk_B, \sk_B)$ for an additively homomorophic encryption scheme and exchange their respective public key $\pk_A, \pk_B$}.
  \end{itemize}
    
    \smallskip
\textbf{Protocol:}
    
\begin{enumerate}
\item Both A and B append dummies to each column $\ell\in [L]$   by sampling from a dummy  space according to Algorithm~2.  %{\color{blue}A and B encrypts their secret values $(v^A_1, \ldots, v^A_m)$ into $(\ct^A_1, \ldots, \ct^A_m)$ and $(\ct^B_1, \ldots, \ct^B_n)$}.

\item
      \begin{itemize}
        \item  A and B separately hash each input column by  $\hash(\mathbf{a}_{\ell} )$ and $\hash(\mathbf{b}_{\ell} )$  and then compute the exponentiation, \ie, $\hash(\mathbf{a}_{\ell} )^{\alpha_{\ell}}$ and 
$\hash(\mathbf{b}_{\ell} )^{\beta_{\ell}}$, for all $\ell\in [L]$.
        \item A and B 
        permute  the order of rows in the hashed and exponentiated  records  with independently uniformly random permutations $\pi_{A_1}: [n]\to [n]$
         and $\pi_{B_1}: [n]\to [n]$, respectively,        and each column is denoted by 
$\hash(\mathbf{a}_{\ell} )^{\alpha_{\ell}}_{\pi_{A_1}}$ and 
$\hash(\mathbf{b}_{\ell} )^{\beta_{\ell}}_{\pi_{B_1}}$, for all $\ell\in [L]$.
         After that, they exchange these records.         
     \end{itemize}
        % 
          
\item 
  \begin{itemize}
    \item      A exponentiates  $\hash(\mathbf{b}_{\ell} )^{\beta_{\ell}}_{\pi_{B_1}}$ with $\alpha_{\ell}$
    for  $\ell\in [L]$ and then permutes the order of rows 
  with independently uniformly random permutation $\pi_{A_2}$ to obtain  
$\mathsf{PII}_{B,\pi}^{\beta\alpha}$, where the $\ell$-th column is denoted by  $\hash(\mathbf{b}_{\ell} )^{\beta_{\ell}\alpha_{\ell}}_{\pi_{B_1}\pi_{A_2}}$.
    Then  A sends the $\mathsf{PII}_{B,\pi}^{\beta\alpha}$  to  B.
    \item    
    B exponentiates  $\hash(\mathbf{a}_{\ell} )^{\alpha_{\ell}}_{\pi_{A_1}}$ with $\beta_{\ell}$
    for  $\ell\in [L]$ and then permutes the order of rows 
  with independently uniformly random permutation $\pi_{B_2}$ to obtain 
$\mathsf{PII}_{A,\pi}^{\alpha\beta}$, where the $\ell$-th column is denoted by  $\hash(\mathbf{a}_{\ell} )^{\alpha_{\ell}\beta_{\ell}}_{\pi_{A_1}\pi_{B_2}}$.
Then  B sends  $\mathsf{PII}_{A,\pi}^{\alpha\beta}$   to  A.
    \end{itemize}
                
        
  \item 
  Iterate over  $\ell=1,\ldots L$:
  \begin{itemize}
  \item
  Party A computes the matching  $\hash(\mathbf{a}_{\ell}[i])_{\pi_{A_1}\pi_{B_2}}^{\alpha_{\ell}\beta_{\ell}}=\hash(\mathbf{b}_{\ell}[j])_{\pi_{B_1}\pi_{A_2}}^{\beta_{\ell} \alpha_{\ell}}$ for all $i\in [m]$, $j\in [n]$ and updates 
$\mathsf{PII}_{B,\pi}^{\beta\alpha}$
  by removing the complete rows   that contain the matched  
  $\hash(\mathbf{b}_{\ell}[j])_{\pi_{B_1}\pi_{A_2}}^{\alpha_{\ell}\beta_{\ell}}$ for all $j\in [n]$.
  for all $i\in [m]$.
  Meanwhile, A appends the removed rows to $\mathsf{PII}_{\cap,A}$.

  \item Party B
computes the matching  $\hash(\mathbf{b}_{\ell}[j])_{\pi_{B_1}\pi_{A_2}}^{\beta_{\ell} \alpha_{\ell}}=\hash(\mathbf{a}_{\ell}[i])_{\pi_{A_1}\pi_{B_2}}^{\alpha_{\ell}\beta_{\ell}}$ for all $j\in [n]$, $i\in [m]$ and updates 
$\mathsf{PII}_{B,\pi}^{\beta\alpha}$
  by removing the complete rows that contain the matched 
  $\hash(\mathbf{a}_{\ell}[i])_{\pi_{A_1}\pi_{B_2}}^{\alpha_{\ell}\beta_{\ell}}$ 
  Meanwhile, B appends the removed rows to $\mathsf{PII}_{\cap,B}$.
  
  \end{itemize}
        % 

 \item Party A and B obtain $\mathsf{PII}$ by individually sorting the rows of $\mathsf{PII}_{\cap,A}$ and $\mathsf{PII}_{\cap,B}$ in descending order of the first column ciphertext.  
    \end{enumerate}
    \end{minipage}
    }

==> protocols/revised_protocol.tex <==
%!TEX root = ../main.tex




==> sections_bak/0-abs.tex <==
\begin{abstract}
To address recent research findings regarding the membership leakage in Private Set Intersection (PSI) protocols, 
stemming from revealed intersection sizes embedded within the PSI execution, 
we present the DPCA-PSI protocol. DPCA-PSI seamlessly integrates a novel \emph{two-party distributed Differential Privacy} (DP) mechanism with a PSI protocol specifically designed to effectively mitigate membership leakage while meeting practical requirements for multi-ID PSI settings.

In multi-ID PSI, where each record is represented by $L$ IDs, the total number of matched ID combinations equals $2^L$, resulting in exponential information leakage for membership inference attacks. To prevent such \emph{cross-ID information leakage}, the designed PSI protocol ensures the independent matching of distinct IDs. Additionally, the corresponding distributed DP mechanism is achieved through a unique dummy pattern design that prohibits the linking of intersections across multiple IDs. Consequently, DPCA-PSI only needs to address a constant membership leakage rate, eliminating the need for dummy overhead used in the DP mechanism even as the number of ID columns increases.
We also conduct meticulous DP accounting for multiple executions of the proposed distributed DP mechanism. Leveraging parameter optimization for DP accounting, we further reduce the size of dummy variables evidently compared to the basic DP composition.

DPCA-PSI has been open-sourced\footnote{Anonymous link: \url{https://github.com/tiktok-privacy-innovation/PrivacyGo/tree/main/dpca-psi} 
}, and extensive experiments across various settings demonstrate its superiority in terms of computational and communication efficiency, as well as user membership protection.
Compared with other PSI protocols with intersection size hidden, DPCA-PSI achieves a computation saving of over $100\times$ for join and compute tasks. This is due to the downstream MPC computation operating only on the intersection rather than on the entire dataset as operated in size-hiding PSI protocols.

% In the era of data explosion, a huge amount of personal data is generated and collected by different entities every day. 
% To make the best use of such dispersed data, the first step will be identifying common entities across datasets owned by different parties. 
% The most efficient approach is pooling all the data and performing analytics over the joined dataset. 
% However, this approach is a clear infringement of not only the commercial interests of data owners but also the privacy of users. 
% Private record linkage (PRL) aims to solve this problem in a secure manner: it allows two mutually untrusted parties to identify which records in their respective private database belong to the same entity without revealing information about other records. 
% Due to its wide applicability and importance, PRL has attracted significant research attention recently. 

% Despite the increasing interest from both academics and industry, so far there is no PRL solution with linear complexity for multi-ID records. \todo{meta's protocols actually have linear complexity}
% In contrast, the single-ID PRL problem can be solved using the well-studied private set intersection (PSI) protocols. 
% In this paper, we propose a novel and efficient protocol for multi-ID record matching between two private databases. 
% Our solution cleverly combines techniques of differential privacy (DP) and PSI to offer strong privacy protection. 
% Our experiment demonstrates the practicality of our construction: the protocol completes in xxx minutes (resp. YYY minutes) when it is executed over two datasets with xxx records in the LAN (resp. WAN) setting. 




\end{abstract}

==> sections_bak/1.1_multi-ID.tex <==
\subsection{Multi-ID PSI: Practical yet Often Overlooked}
\label{sec:intro-multi_id_psi}
If the data records of each entity only contain a single identifier, say email address, and further assuming that we are only interested in~\emph{exact matching} records, the private-preserving matching problem is the well-known PSI problem in the literature. 
Although much effort has been devoted to the research of PSI protocols and significant progress has been made in the construction of efficient PSI protocols, multi-ID matching is relatively understudied in the PSI literature. 
This is a sharp contrast to the real-world applications, in which records are often indexed by multiple IDs, such as phone number, email address, IP address~\etc, because different parties rarely share one type of identifier that uniquely identifies each user.
Employing an exact equality check for matching two records from different entities using a single ID column may result in missing a significant number of records in the final result. In practice, the use of multi-ID PSI is often necessary, yet it is a topic that is rarely explored in academic research.

Note that the existence of numerous identifiers facilitates adaptable join logic defined by the business requirements in practice and frequently results in {\it many-to-many } connections. For instance, Party A and Party B might both depict individuals through email and phone numbers. Nevertheless, a user of Party A could employ different emails during the purchase without updating them on Party B's platform.

A commonly employed multi-ID matching logic is the \textit{waterfall matching}, a ranked deterministic join logic~\cite{multi_key_meta}.  The {order} of identifiers is established through mutual agreement between the parties involved in the matching process. In the initial round, all records are exclusively matched based on the first identifier, resembling a single-key matching approach. Subsequently, in a second round, matching is carried out on the second identifier, limited to records that remained unmatched in the preceding round. This iterative process continues as many times as the maximum number of identifiers present in the records.
Note that this waterfall matching logic solves the many-to-many matching uncertainty problem and is widely used in practice, such as in ad measurement~\cite{multi_key_meta}.


One approach to achieving multi-ID waterfall PSI involves invoking the single-ID PSI protocol on distinct ID columns and subsequently combining the outputs of these PSI protocols. However, as each ID's matching depends on the outcomes of preceding ID columns, it becomes expensive to evaluate the matching procedure itself via general MPC with equality checks, which are used to decide whether the data has already been matched. Unfortunately, the resulting general MPC protocol is prohibitively costly in communication and computation for real-world business scenarios.




%Figure 1 further reinforces the claim that multi-ID PSI is more prone to membership attacks. Fig.~1 also verifies the claim that the multiple-ID PSI is more vulnerable to membership attacks.
%












% One may try to further reduce this leakage by using so-called~\emph{circuit PSI}. 
% Circuit PSI is a variant of PSI, whose output is not the intersection in plain, but secret shared across the two parties.
% Therefore, the output is of circuit PSI can be fed directly to subsequent MPC protocols for secure data analytics. 
% While this %further improvement 
% approach seems to work at a high level, there are technical difficulties to be solved. 
% To the best of our knowledge, all efficient circuit PSI constructions~\cite{popets/ChandranGS22,eurocrypt/Pinkas0TY19,cans/KarakocK20} so far rely on the~\emph{Cuckoo hashing} paradigm, which maps the secret shares of the intersection into a (Cuckoo) hash table. 
% As a result, the ordering of the intersection of each ID column will be different. 
% We could align the ordering of each column intersection secret shares using an~\emph{oblivious shuffling} protocol, but the state-of-the-art asymptotic complexity of such protocol is $O(n \log n)$, which is quite inefficient.  

==> sections_bak/1.2_size-reveal.tex <==

\subsection{\jd{The Meaning of Membership Leakage in PSI}}
\label{subsec:size}

We provide an in-depth discussion of the potential privacy risks linked to membership leakage in size-revealing PSI
using the ad measurement example mentioned earlier. Recall that the advertiser and the publisher join their datasets of user identifiers to perform PSI.
If a user opts out of tracking on the ad publisher's end (for example, by turning on the ``ask app not to track'' setting on iOS for the publisher's app), the publisher cannot associate the user's activity on their app with the user's data on any third-party platform, including the user's purchase data on the advertiser's side. 
% Since then, the ad industry has relied on ECDH-style PSIs to perform ad measurement without sharing unencrypted data with each other~\cite{google-advertising, PS3I}. However, as explained above, those protocols suffer from membership leakage, which could induce privacy and business risks for both advertisers and ad publishers. 
%Below, 

We present two scenarios illustrating how the membership information on the advertiser's side can be exploited by the publisher, leading to privacy and business risks. Note that similarly, the advertiser can also act as a curious attacker, attempting to infer the membership of its users on the publisher's side.
\begin{itemize}[leftmargin=*]
\item \textbf{The publisher learns who, denoted by $x$, is in his set $A$ but not in the advertiser's set $B$, \ie, $x\in A\setminus (B\cap A)$.} In this case, the ad publisher can identify users on its platform who viewed an ad but did not make purchases at the advertiser's end. This constitutes a leakage of confidential information, as the advertiser may not want the ad publisher to gain access to such details, especially as they could be valuable for the advertiser's competitors.
    \item \textbf{The publisher learns who, denoted by $x$, is in his set $A$ is also in the advertiser set $B$, \ie, $x\in A\cap B$.} In this scenario, the ad publisher is able to learn the activity of the identified user (\ie, someone who made a purchase) on the advertiser's side. This situation constitutes a privacy breach, particularly if the user has opted out of tracking. Furthermore, from the advertiser's perspective, they would not want the ad publisher to possess the capability to identify their clients.
\end{itemize}

\subsection{\jd{Assessment of Membership Leakage in PSI}}

\begin{figure*}[t]
\centering 
\subfigure[\% of membership leakage in single-ID PSI]
{\includegraphics[width=0.31\textwidth]{images/singleid1.pdf}
\label{fig:singleid_leakage}}
\subfigure[\% of membership leakage leakage in 4-ID PSI]
{\includegraphics[width=0.31\textwidth]{images/multi-id.pdf}
\label{fig:multiid_leakage}}
\caption{Percentage of user membership leakage versus execution numbers of the size-revealing PSI protocols. We consider PSI-sum~\cite{google-psi} for single-ID PSI on the l.h.s. and multi-ID PSI~\cite{multi_key_meta} on the r.h.s. with $4$ IDs under recently proposed membership inference attacks in Guo et al. USENIX 22'~\cite{Guo2022birds} and Jiang et al. NDSS24'~\cite{Bo}. It shows that the membership leakages for both cases follow a linear trend. Additionally, the results reveal that multi-ID PSI is more susceptible to membership inference attacks, exhibiting higher membership leakage under the same PSI execution times compared to single-ID PSI.
    These attacking techniques have also been applied to assess our proposed DPCA-PSI protocol, which demonstrates no leakage with $\epsilon = 2$.}
\vspace{-12pt}
\label{fig:psi_leakage}
\end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\textwidth]{images/PSI_leakage.png}
%     \caption{Percentage of user membership leakage versus execution numbers of the size-revealing PSI protocols. We consider PSI-Sum~\cite{google-psi} for single-ID PSI on the left-hand side and multi-ID PSI~\cite{multi_key_meta} on the right-hand side with $5$ IDs under recently proposed membership inference attacks in Guo et al. USENIX 22'~\cite{Guo2022birds} and Jiang et al. NDSS24'~\cite{Bo}. It shows that the membership leakages for both case follow a linear trend. Additionally, the results reveal that multi-ID PSI is more susceptible to membership inference attacks, exhibiting higher membership leakage under the same PSI execution times compared to single-ID PSI.
%     These attacking techniques have also been applied to assess the security of our proposed DPCA-PSI protocol, which demonstrates no leakage due to the specific designed DP protection with $\epsilon = 2$.}
%     \label{fig:psi_leakage}
% \end{figure*}

%To set the stage for introducing our privacy-protecting solution differentially-private cardinality PSI (DPCA-PSI), we will initially examine the feasibility and effectiveness of leveraging the intersection size to conduct a membership inference attack, as shown in~\cite{Guo2022birds, Bo}.
We first examine the feasibility and effectiveness of leveraging the intersection size to conduct a membership inference attack.
Consider a scenario where one party in the PSI protocol is interested in determining whether the $m$ users in their set belong to the other party's set. In a brute force attack, the curious party straightforwardly manipulates their own set by adding or removing a single record corresponding to one user/identifier. By observing the difference in intersection size between two executions of a size-revealing PSI protocol, the attacker can tell whether the modified user/identifier belongs to the other party's set or not. Although this attack is slow with a complexity of $\mathcal O(m)$, it demonstrates the feasibility for such membership leakage. 

Guo~\etal~\cite{Guo2022birds} proposed an efficient attack on size-revealing PSIs using a binary-search-like strategy. They construct a binary tree where each node contains a non-empty set. Employing depth-first search (DFS), the attacker systematically explores the tree, invoking the PSI protocols during each iteration to infer set membership. The process identifies subsets containing target elements and determines non-membership for others. This technique %shows its ability to 
reduces the complexity required to ascertain users' membership from $\mathcal O(m)$ to $\mathcal O(\log m)$, highlighting a privacy breach in size-revealing PSI protocols.
In a follow-up study, Jiang~\etal~\cite{Bo} suggested optimized hierarchical structural attacks. 
Instead of uniformly dividing all nodes in the binary tree, they propose to use an uneven tree partition strategy based on dynamic programming and %. Their findings 
show that the algorithm is optimal for maximizing the number of expected membership inferences within the context of an uneven tree structure. 
% \donghang{a bit unclear here}Despite the randomness in the tree construction for searching the attacking strategy, Jiang~\etal~\cite{Bo} demonstrated that even in the worst-case scenario of tree partition for attacking, membership leakage cannot be overlooked.

\jd{Note that effective membership protection against size-revealing PSI remains unresolved, despite the observation of membership leakage in recent studies \cite{Guo2022birds, Bo}.} 
Fig.~\ref{fig:singleid_leakage} illustrates the membership leakage during multiple executions of the size-revealing PSI protocol between Party A and B, with a curious party employing the membership inference attack proposed in prior work~\cite{Guo2022birds, Bo}. We utilized the size-revealing PSI protocol from~\cite{google-psi}. This curious party precisely follows the pre-specified size-revealing PSI protocol, while utilizing intersection size to determine whether the curious party's users are members of the other party. Without loss of generality, let's assume the curious attacker to be party A. Using the attack methods in prior work~\cite{Guo2022birds, Bo}, when the size-revealing PSI protocol is executed $20$ times, over $2.5\%$ of users' membership information is leaked.

\textbf{The multi-ID may be more vulnerable to membership attacks.}
    When managing multi-ID records, a size-revealing PSI protocol could also reveals the sizes of all subsets within the multi-IDs~\cite{multi_key_meta} (\eg, the attacker knows how many records share the same values on both the first and the second ID under semi-honest security model). If each record is represented by $L$ IDs, the total number of the subsets of IDs equals $2^L $, which experiences exponential growth with the value of $L$. Therefore, \emph{the cross-ID intersection size number grows exponentially}, causing rapid privacy loss. 
    We also conduct experiments using multi-ID PSI protocols following the same setting as before, assuming that each user has 4 different IDs. We utilized the size-revealing PSI protocol from~\cite{multi_key_meta} for the multiple ID case.
%The left figure in Fig.~\ref{fig:psi_leakage} depicts the privacy leakage for users in Party A under the scenario where both participating parties use single IDs, while the right figure represents the case where s. As the membership inference method only requires intersection size information, it has the same inference capability across all size-revealing PSI scenarios. 
After $20$ PSI executions, the number of leaked users exceeds $6\%$ as shown in Figure~\ref{fig:multiid_leakage}.









==> sections_bak/1.3-contribution.tex <==
\subsection{Our Contributions}
We propose the Differentially Private Cardinality PSI, the DPCA-PSI protocol.
DPCA-PSI is designed to support multi-ID PSI and incorporates a newly devised two-party DP mechanism to address membership leakage issues for both parties simultaneously. Our contributions can be summarized as follows:

\noindent{\jd{\textbf{Two-party  computational DP mechanism compatible with PSI computation.} 
The prevailing central DP and local DP methods described in the literature typically involve either the aggregator or the local user adding random noise for DP protection. That means that they cannot be used for PSI protocols that do not have an aggregator. For the first time, we introduce a two-party DP approach integrated into the secure computation protocol, ensuring that the revealed intersection size is under a dual-sided computational DP. As a result, this DP mechanism seamlessly integrates into the existing literature on single-ID size-revealing PSI with simulatability-based security proof.}}
Our experiments %findings 
suggest that, after synergizing with the novel two-party DP mechanism, PSI's membership leakage, initially characterized by a linear leakage rate, is effectively eliminated, achieving leakage-free status under reasonable DP parameters,~\eg, $\epsilon =2$. This improvement is achieved with a small %amount of 
communication\&computation overhead for large-scale PSI problems.

\noindent\textbf{DPCA-PSI eliminates exponential membership leakage rate, irrespective of the number of IDs.}
\jd{Protecting the exponential growth of membership information leakage associated with multiple IDs introduces an exponential communication and computation complexity growth rate due to the extra dummy required.
To eliminate the exponential rate leakage w.r.t. multiple IDs, we design the multi-ID PSI in DPCA-PSI to ensure the independence of distinct ID matching, preventing any cross-ID information leakage.  This ensures that membership leakage rate remains constant as the number of IDs increases, eliminating the necessity for dummy overhead to counteract exponential privacy loss rates.}

\noindent\textbf{Enhancing tight DP accounting to minimize dummy size in multiple executions of DPCA-PSI.} In multiple runs of the DPCA-PSI protocol in practice, we offer an FFT-based numerical accounting assessment to evaluate tight $(\epsilon, \delta)$-privacy loss using the privacy loss distribution. %By leveraging
We optimize parameters in the accounting process by theoretical analysis, mitigating the impact of dummy variables on additional communication and computational costs in the PSI protocol.

% \noindent\textbf{Rigorous security proof.} The DPCA-PSI protocol integrates the strengths of both MPC and DP. For security analysts, we provide rigorous security proof for the proposed computational setting based on simulation-based definitions. 

% \noindent\textbf{Experiments.}We implement DPCA-PSI and conduct extensive experiments across various bandwidth scenarios. The results demonstrate that DPCA-PSI surpasses existing multi-ID PSI protocols in computation, communication efficiency, and user membership protection.

\subsection{Paper Outline}
% Since the view of a size-revealing PSI protocol contains the following information:
% (1) intersection size information;
% (2) the generated randomness during the protocol execution; and
% (3) the messages received from the other party.
We provide an example to illustrate the workflow of the DPCA-PSI protocol in Section~\ref{sec:example}. In the following sections, we delve into the specifics.
In Section~\ref{sec:dp}, we illustrate how our specifically designed mechanism achieves DP intersection size in the distributed setting for both single-ID and multi-ID PSI.
In Sections~\ref{sec:dpca-psi}, we provide details of the MPC protocol constructing DPCA-PSI and the corresponding security proof under simulation-based computational DP~\cite{crypto/MironovPRV09}. In Section~\ref{sec:dpca-psi-payloads}, we demonstrate that DPCA-PSI is compatible with downstream MPC tasks.
Finally, in Section~\ref{sec:experiments}, we evaluate DPCA-PSI by conducting extensive experiments across various settings.

==> sections_bak/10_conclusion.tex <==
\section{Conclusion}

In this paper, we present the DPCA-PSI protocol as a solution to address the challenge of membership leakage arising from revealed intersection sizes during PSI execution. By integrating a novel two-party distributed Differential Privacy (DP) mechanism with a specially designed PSI protocol, DPCA-PSI effectively mitigates membership leakage while satisfying practical requirements for multi-ID waterfall matching.
The protocol is specifically tailored for multi-ID PSI scenarios, preventing potential exponential information leakage for membership inference attacks with respect to the number of IDs.
We demonstrate the effectiveness of DPCA-PSI through extensive experiments conducted in various settings, highlighting its superiority in terms of computational and communication efficiency, as well as robust protection of user membership. 

% For example, as illustrated in Table~\ref{tbl:benchmark_with_payload_single_id}, compared with other size-hiding PSI protocols, our method achieves a computation saving of $100\times$ for join and compute tasks. This is due to the downstream MPC computation operating only on the intersection, rather than on the entire datasets as done in size-hiding PSI protocols.

% In this paper, we present DPCA-PSI, a two-party multi-ID PSI protocol with differential privacy guarantee. It effectively mitigate membership leakage in multi-ID PSI settings, and provide differential privacy protection to PSI results.

==> sections_bak/1_introduction.tex <==
%!TEX root = ../main.tex

\section{Introduction}
\label{sec:1}
Privacy-enhancing technologies (PETs) have attracted growing attention from researchers, practitioners, and governments worldwide~\cite{Whitehouse}, offering the potential to advance data-driven technologies such as Artificial Intelligence and Machine Learning, while safeguarding privacy. Despite the acknowledgment of PETs by governments and privacy regulatory bodies (\eg, the UK ICO published guidelines recognizing PETs' ability to comply with privacy by design), PET as well as the application of PET in practice continue to demand active research. 

Among the notable PETs is secure multiparty computation (MPC), which enables involved parties to gain useful insights from sensitive data without accessing the underlying information. As a specialized MPC protocol, private set intersection (PSI) %is a technique used to 
computes the intersection of datasets from multiple parties without disclosing any information beyond the intersection. Downstream computation can also be performed on the resulting \jd{encrypted intersection set and its associated payloads} using general-purpose MPC protocols~\cite{patra2021aby2,yao1986generate,GMW87} for statistical analysis. This process is often known as \textit{PSI and Compute} (or similarly Private Join and Compute)~\cite{google-psi}.

\textbf{Practice requires PSI and Compute:} A practical application of \textit{PSI and Compute} is to measure the effectiveness of digital advertisements. Advertisers launch an ad campaign on publishers' platforms and want to understand whether users engaging with these ads eventually make a purchase. The data needed to compute the effectiveness of the ad campaign is typically split between the ad publisher and the advertiser. 
The ad publisher holds identifiers for users who viewed the advertising campaign, while the advertiser holds identifiers and \jd{payloads} representing the amount spent on purchases by users. Challenges arise as users opt out of sharing individual data for advertising purposes through disabling tracking features on \jd{iOS or Android devices}~\cite{NYT2021Tracking,Forbes2022Cookies}. Ad publishers and advertisers may no longer join their raw data, which often contains individual user records. 

Consequently, the ad industry has turned to \textit{PSI and Compute} for ad measurement in order to compute the statistics without %the need to 
sharing unencrypted data between the two parties~\cite{google-advertising, PS3I}. Throughout this process, all identifiers and associated data remain fully encrypted and unreadable. This approach ensures that neither party needs to disclose their raw data, yet they can compute aggregate statistics, such as the total purchase amount resulting from an ad campaign.

\textbf{Size-revealing PSI inadvertently discloses input membership:}
A variety of \textit{PSI and Compute} protocols \jd{under semi-honest security model} have been developed in academia and deployed in the industry. In particular, ECDH-PSI protocols~\cite{meadows1986more, ion2020deploying, bhowmick2021apple,meta-password, multi_key_meta} are the most common in the industry due to their ease of use and capacity to handle large datasets with low communication overhead. Additionally, it is better suited for practical needs such as accommodating multi-ID matching~\cite{multi_key_meta}. {\jd{Multi-ID matching pertains to scenarios where the datasets involved in PSI contain multiple types of identifiers, such as emails and phone numbers, allowing for fuzzy matching to enhance the match rate. }}

It is worth noting that ECDH-PSI, while keeping all data encrypted, discloses the size of the intersection set during protocol execution. We refer to such protocols as {\it size-revealing PSI}, which also include PSI protocols constructed through other cryptographic primitives such as homomorphic encryption and oblivious pseudorandom function. Recent studies~\cite{Guo2022birds,Bo} have found that \jd{adversaries who adhere to the  protocol can exploit size-revealing PSI to de-anonymize specific data records in the input sets}, thereby leaking membership information about the input sets. 
While this does not directly break the original security model of the PSI protocol, which aims to keep each party's input set confidential, such PSI can divulge additional information about {\it{whether members of one set belong to the other set or not}}. As a result, this membership leakage could give rise to privacy risks. \skz{Even though there exist PSI protocols that do not disclose intersections sizes, such as Circuit PSIs, they are not currently applicable in multi-ID use cases.}

In the following, we describe the privacy leakage of size-revealing PSI. We then explore how this leakage could be exploited to conduct a membership inference attack and discuss how this attack might be aggravated by the practical settings of multi-ID PSI.

% In the age of data analytics, organizations gather large amounts of data for various purposes. 
% For instance, research institutes may acquire patient data for medical studies, while Internet companies collect customer data to offer targeted suggestions. 
% As a result, individuals' digital profiles are spread across different data collectors. 
% However, it is common knowledge that the effectiveness and accuracy of machine learning algorithms improve considerably with more high-quality training data. 
% To fully unlock the power of data analytics, it is essential to gather information from various parties and conduct analytics across the joint data set.

% Despite the technical benefits, cross-organizational data sharing comes with several immediate practical obstacles. 
% Firstly, organizations may not trust each other and may not be willing to share their data with other parties, particularly when the data has considerable commercial value. 
% Secondly, even if two organizations agree to collaborate and share data, it may still be subject to privacy regulations, such as GDPR, particularly when the two organizations operate in different jurisdictions. 
% In fact, such regulations still restrict intra-company data transfers across countries.

% To address the concerns of regulatory bodies and also respect the financial interests of participating data owners, researchers have proposed to apply various privacy-enhancing technologies, \eg, secure multi-party computation (SMC), differential privacy (DP), homomorphic encryption (HE), to the data sharing pipeline. 
% Prominent examples include Google's advertisement measurement protocol~\cite{ion2020deploying} using~\emph{private set intersection} and Apple's differential privacy implementation in their data collection system~\cite{appleDP}. 


% %\subsection{Privacy-preserving record linkage}
% Linking records between two databases is an essential step in the data analytic pipeline. 
% If we disregard privacy concerns, linking records can be done easily by comparing all records directly. 
% Privacy-preserving record linkage (PPRL)~\cite{acns/AdirADKMMS22,sp/ChristenRS20,popets/ArmknechtHS23,ccs/HeMFS17} aims to provide a strong level of privacy, ensuring that unlinked records remain hidden and no information is disclosed. 
% PPRL is especially useful in applications where two databases contain overlapping IDs that are stored in mutually untrusted parties. 
% For instance, two companies may want to find common customers before launching a joint promotion, or two hospitals may seek to merge their patient data for medical research purposes. 
% In both cases, sensitive data and IDs in the databases need to be safeguarded, particularly data that will not be used in the final analysis (\ie, records not in the intersection). 
% The straightforward approach of comparing records directly is not appropriate for these settings. 



\input{sections/1.2_size-reveal}
\input{sections/1.1_multi-ID}
\input{sections/1.3-contribution}

\section{An Illustrative Example of DPCA-PSI}
\label{sec:example}
\jd{
We present a specific illustrative example of DPCA-PSI, as shown in Fig.~\ref{fig:DPCA-PSI-A} and Fig.~\ref{fig:DPCA-PSI-B}. Further analytical details and security proofs are provided in subsequent sections.
In this example, each data sample in Party A and Party B is represented by three IDs. It is important to note that in practical scenarios, different IDs often originate from independent subspaces, such as email addresses, phone numbers, and IP addresses. Therefore, they are disjoint from each other. In the following, we explain how DPCA-PSI works.}

\jd{A common set of dummy IDs with $2\tau$\footnote{The quantity $\tau$ is determined by the total DP budget according to our DP analysis as shown in the next section.} rows is generated for both parties using a pseudorandom generator with a shared seed locally. It's important to note that each column of dummy IDs is disjoint from each other and from the input IDs. This is achieved by random sampling from disjoint subspaces. For instance, dummy IDs could be sampled from both lowercase and uppercase letters of the Greek alphabet, as well as Roman numerals as shown in Fig.~\ref{fig:DPCA-PSI-A}. In practice, there are numerous methods to ensure that dummy IDs are sampled from disjoint subspaces.}

\jd{Each party independently conducts a random local shuffle of each dummy column, selecting the first $\tau$ elements as the dummy and appending them to their respective actual input column but different rows to make sure the DP mechanism for each column are independent. These $\tau$ rows for each column are denoted in purple and blue colour in Fig.~\ref{fig:DPCA-PSI-A}.
The remaining portion of each column is filled with additional stand-in elements, which are distinct from all the dummy elements. Additionally, the stand-in elements for different columns are also disjoint, as indicated by the radial gradient pattern in Fig.~\ref{fig:DPCA-PSI-A}.
}

\jd{
The parties utilize an ECDH-style PSI protocol to identify common elements in the first column.
We enhance the ECDH-PSI protocol by introducing a random permutation to prevent either party from knowing which specific rows are matched in a given round.
Subsequently, both parties eliminate the intersection rows from the other party's "encrypted" input sets following the waterfall matching logic, which is detailed in Section~\ref{sec:intro-multi_id_psi}. }

\jd{Both parties then conduct single-ID PSI for the next column using the same logic (as depicted in Figure~\ref{fig:DPCA-PSI-B}).
It is important to note that the protocol for the first column differs from the protocol for the subsequent columns.
The inputs for PSI in the first column are the plaintext of their own input sets. However, upon completion of the PSI for the first column, each party possesses the other party's remaining "encrypted" input sets to use as input for the subsequent PSI.
As a result, additional steps are necessary for these columns, such as removing one layer of "encryption" (i.e., exponentiation) while applying another layer of "encryption" (as depicted in Step 5) to facilitate blind matching.
Distinct "encryption keys" (i.e., exponents) are necessary for each column to prevent cross-column information leakage, thereby mitigating the risk of exponential membership disclosure.}

\jd{Finally, each party acquires the encrypted matched IDs following the waterfall matching logic. The matched size of each column is randomized by the dummy variables, a formal demonstration of which will be provided in the next section, ensuring dual-sided DP guarantee.
For downstream tasks, one could customize the payload associated with the dummy according to specific applications and requirements. For instance, in PSI-sum~\cite{google-psi}, setting the dummy's payload to 0 wouldn't affect the final sum accuracy. Additionally, one could even design additional MPC-based secure additive noise generation~\cite{mpc_noise_ccs23, Schneider-noise} to ensure downstream results under DP, though this is beyond the scope of this paper.}



\begin{figure*}[htbp!]
    \centering
\includegraphics[width=\textwidth]{images/AnonPSI-A.png}
    \caption{An illustration of DPCA-PSI (Part 1)}
    \label{fig:DPCA-PSI-A}
\end{figure*}

\begin{figure*}[htbp!]
    \centering
\includegraphics[width=\textwidth]{images/AnonPSI-B.png}
    \caption{An illustration of DPCA-PSI (Part 2)}
    \label{fig:DPCA-PSI-B}
\end{figure*}



% % \subsection{Singling out in the GDPR}


% % \subsection{what does protection individuals mean in PSI}



% \subsection{Challenges}





% TBD
% {\textbf Intersection Revealed}

% {\textbf Intersection NOT Revealed}  protect unmatched data, intersection is disclosed to one party or both parties

% Circuit based: intersection is NOT disclosed to any party

% HE: not communication/computation efficiency. cardinality disclosure.
% One solution in~\cite{kacsmar2020differentially} is to compute the intersection  based on homomorphic encryption (HE) and then apply  DP mechanism to protect the result. This way it will be hard for one party to determine if a single data belongs to the other party or not based on the result.  However, it is well known that compared with other cryptographic approaches fully homomorphic encryption incurs expensive operations and large communication cost due to added noise.  


% {\textbf Differential Privacy Integrated PSI}
% The idea of differentially-private over-estimates of
% the true bin load has been used previously in the context
% of PSI (and private record linkage) protocols~\cite{groce2019cheaper}. These protocols accelerate the PSI however, do not offer a DP protected intersection result.




% \noindent\textbf{}

% \noindent\textbf{attributing aggregate ad conversions
% }

% The advertiser pays the advertising provider, such as a website owner/search engine, to put their ad in areas that are not directly related to the ads supplier's own content. People would make a purchase from the marketer after watching an internet advertisement.

% As a result, the advertiser would like to know statistics regarding the online advertising campaign, such as customer quantile ages.
% The required information, on the other hand, is controlled separately by the ad supplier, who knows which people have viewed a given ad and their features, and the advertiser, who knows who made a purchase.

% Regardless of whether either party is reluctant or unable to disclose the underlying data, both would prefer to compute an aggregate population-level privacy preserved statistic, such as how many people viewed an ad and then made a corresponding purchase, and how much those users spent in total. Their goal is to accomplish this while assuring that no personally identifying information about individual users can be derived from the released statistics.


% \medskip
% \noindent
% \textbf{Symbols:}
% In the following, we use uppercase letter, e.g., $X$, to denote a random variable and lowercase $x$ to denote a constant.
% We define an indicator   ${\mathbbm 1}_{\mathcal A}(a_i)$ to represent whether an element $a$ is in the  $\mathcal A$ or not, i.e.,
% \begin{equation}
% {\mathbbm 1}_{\mathcal A}(a)\triangleq 
% \left\{
%              \begin{array}{lr}
%  1,  & \textrm{if} \quad a\in \mathcal{A}, \\ 
% 0, &\textrm{if} \quad a\notin  \mathcal A.
%              \end{array}
% \right.
% \end{equation}

% % \begin{table*}[h]
% %     \centering
% %     \caption{ Notations used throughout the paper.}
% %     \begin{tabular}{cc}
% %     \toprule
% %     % $\mathcal{U}$     &  Unique identifier set \sz{replace with a more general $\bin^*$?}\\
% %     ${A}=[a_1,...,a_n]$     &  Alice's unique identifier set (size $n$)\\
% %     ${B}=[b_1,...,b_n]$     &  Bob's unique identifier set (size $n$) \\
% %   $\mathsf{S}(A; p)$&\\
% %     $(\epsilon_a, \delta_a)$ \quad
% %     $(\epsilon_b, \delta_b)$ & \\
% %     $\mathcal{X}=\{x_{f,1},...,x_{f,n}\}^F_{f=1}$ & Bob's payload (size $|F|\times n$)\\
% %     $\mathcal{I}\triangleq\mathcal{A}\cap\mathcal{B}$     &  The intersection set\\
% %     $\mathcal{I}_\textrm{DP}\triangleq\mathcal{M}(\mathcal{A},\mathcal{B})$     &  The DP protected  intersection set\\
% %     $\alpha, \beta$ & Alice and Bob's secret key, separately\\
% %     $h(\cdot)$ & An analytic function (e.g. sum, median)\\
% %     $\GG, m, g$ & Diffie-Hellman Group with order $m$ and generator $g$\\
% %     $(\epsilon, \delta), \mathcal{M}, \mathcal{D}, \mathcal{O}$ & DP parameters + mechanism + database + output space\\
% %     $\Pr(\mathsf x = x)$ & The probability value that  $\mathsf x = x$. All r.v. will be denoted in sans-serif fonts,\\ & and  the values of such variables in standard font.\\
% %     $\hash(\cdot)$ & Hash function (Note that this is not necessarily to be a random oracle)\\
% %     $S_m$ & The set that includes all possible permutations of $[1,...,m]$ \\
% %     \bottomrule
% %     \end{tabular}
% % \end{table*}




==> sections_bak/2-related.tex <==
\section{Related Works}
% Traditional PSI delves into the methodology through which two or more parties can collaboratively compute the intersection of their respective private input sets. The primary objective is to reveal shared elements within the intersection while preserving the privacy of elements exclusive to each party~\cite{??}.
% This paper directs our focus towards the challenges presented by various applications, such as advertising measurement~\cite{google-advertising} and vertical federated learning~\cite{jiang2022comprehensive}, which rely on additional computations based on the results of the two-party intersection.

% The privacy concern extends beyond determining the membership status of input elements exclusive to each party; it also encompasses those belonging to the intersections. In essence, our emphasis lies in safeguarding the privacy of both the membership status—regardless of whether a data record belongs or does not belong to the intersection.
% We coin this concept as "private join and compute." For example, in~\cite{google-psi}, the idea of "private join and compute" let two parties, each with their own input file, secretly figure out the sum of values for records that shared common identifiers within the intersection.
% We focus on the PSI protocol design and extend this concept to include any computation based on intersections, not necessarily limited to summation.

PSI has been studied extensively in a long sequence of works~\cite{chen2017fast,pinkas2014faster,kolesnikov2016efficient,freedman2004efficient,google-psi,PS3I,multi_key_meta,eurocrypt/Pinkas0TY19,popets/ChandranGS22,eurocrypt/Pinkas0TY19,cans/KarakocK20, pkc/0005DP21,crypto/GhoshS19,access/ZhangCL21, ion2020deploying} using different cryptographic techniques, such as oblivious polynomial evaluation (OPE)~\cite{freedman2004efficient}
, oblivious pseudorandom functions (OPRF)~\cite{kolesnikov2016efficient}
, oblivious transfer~\cite{pinkas2014faster}
, elliptic curve crypto, and homomorphic encryption (HE)
~\cite{chen2017fast}.
%, have been used to construct PSI protocols, offering different trade-offs. 
Additionally, numerous PSI variations, including PSI-Cardinality, PSI-Sum~\cite{ion2020deploying,crypto/MiaoP0SY20}, threshold-PSI~\cite{csfw/HallgrenOS17,pkc/0005DP21,popets/ZhaoC17,crypto/GhoshS19,access/ZhangCL21,wpes/0001C18}, circuit PSI~\cite{popets/ChandranGS22,eurocrypt/Pinkas0TY19,cans/KarakocK20,le2019two}, among others, are shown to be very useful for many real-world applications.

Nonetheless, recent studies~\cite{Guo2022birds,Bo} have highlighted a potential vulnerability in Private Set Intersection (PSI) protocols. If the intersection size is disclosed during the protocol execution, a curious party can exploit this information for a membership inference attack, revealing over 1\% of its data membership—whether it belongs to the intersection or not. This not only poses a privacy risk but also raises concerns about business confidentiality, as detailed in Section~\ref{subsec:size}.
Consequently, we categorize PSI protocols into two groups: size-revealing PSI and size-hiding PSI, based on whether the protocol discloses the intersection size.


\noindent\textbf{Size-revealing PSI:}
Many PSI variants reveal the size of the intersection. For example, PSI-Cardinality only discloses the size of the intersection set without revealing the specific elements within the intersection set. Similarly, other variants like PSI-Sum~\cite{ion2020deploying,crypto/MiaoP0SY20} and threshold PSI~\cite{csfw/HallgrenOS17,pkc/0005DP21,popets/ZhaoC17,crypto/GhoshS19,access/ZhangCL21,wpes/0001C18} also expose the size of the intersection set as part of the protocol output. In certain PSI constructions, as observed in~\cite{le2019two}, the intersection size is shared with both parties to enhance protocol efficiency. \skz{ The disclosure of the intersection set size is regarded as the protocol's intended output, which, however, could inadvertently pose privacy risks in practical scenarios.}


 
 % demonstrate that if we allow multiple PSI invocations on the same input sets of one party, the other party gains even more power and can recover the set membership information only after a small number of queries with curated input sets. The underlying concept here is that the size of the intersection implies the similarity between the sets of two parties. Consequently, one party can extract information about the other party's set by constructing different input sets and assessing the similarity between them. This leakage of membership information can have a significant influence, particularly when the target set contains sensitive information, such as in the context of COVID-19 contact tracing.

\noindent\textbf{Size-hiding PSI:} 
\skz{Circuit PSI, a variant of PSI, generates an output that is not the plaintext intersection but rather a secret shared result across all inputs from both parties. While effective in concealing intersection size, Circuit PSI
faces practical challenges for multi-ID matching, especially with specific logics such as waterfall matching. Currently, no Circuit PSIs support multi-ID, which remains an open research area. }

\skz{Despite its impracticality for multi-ID scenarios, circuit PSI remains less efficient than our proposed PSI, even for single ID matching.}
To date, all efficient circuit PSI constructions~\cite{popets/ChandranGS22,eurocrypt/Pinkas0TY19,cans/KarakocK20} rely on \emph{Cuckoo hashing}, a technique that maps the secret shares of the intersection into a (Cuckoo) hash table. Consequently, the ordering of the intersection within each ID column varies. While it might be feasible to align the ordering of each column's intersection secret shares using an \emph{oblivious shuffling} protocol, the current state-of-the-art asymptotic complexity for such a protocol is $O(n \log n)$, making it considerably inefficient when compared to our proposed PSI with linear complexity.

% Another defense~\cite{Guo2022birds} is to limit the number of PSI invocations with the same input set. 
% However, it remains unclear how to choose the threshold number properly as there are many factors that affects the attacker's efficiency. 
% A small threshold also hurts the utility, although it provides stronger privacy. 
% Another approach is to audit the other party's input set, as the attacks detailed in~\cite{Guo2022birds, Bo} typically construct input sets with specific patterns. 
% If these patterns are identified, the honest party can abort the protocol. 
% Nevertheless, this method is ad-hoc, and it is impractical to recognize and detect all potential attack patterns systematically.

Kacsmar \etal~\cite{eurosp/KacsmarKLNSSBSO20} 
introduce a solution wherein they employ Differential Privacy (DP) mechanisms to protect the cardinality of single-ID Private Set Intersection (PSI) in a client-server scenario. Consequently, only central DP is necessary, as the DP guarantee is specifically essential for the client side. However, in our context, where each party is inquisitive about membership and there is a potential for membership attacks, the application of central DP is not suitable. Instead, a distributed DP approach is required.

Private-ID~\cite{multi_key_meta} is the only publicly available solution for multi-ID matching and computation (with membership leakage). However, it has a drawback: each party can know the intersection size of any subset of IDs, leading to exponential leakage of membership information. \skz{The recent paper by Mouris et al.~\cite{delegated_matching_meta}, within Private-ID~\cite{multi_key_meta}, proposes delegates to extend the traditional two-party protocol to involve one party and multiple smaller parties. There are two key distinctions from our work: (1) \cite{delegated_matching_meta} remains susceptible to membership leakage at the delegates due to their knowledge of intersection sizes, whereas our intersection sizes are DP-protected; (2) our method confines downstream MPC computation to the intersection, while \cite{delegated_matching_meta} accounts for Party C's entire dataset (by setting the secret share of non-intersecting elements to zero). In real-world applications, the intersection typically constitutes less than 1\% of the incoming dataset, underscoring our method's efficiency.}



==> sections_bak/2_problem_formulation.tex <==







% \begin{figure*}[tp]
%    \centering
%    \label{Alg:DPSetIntersection-temp}
%    \input{protocols/main_protocol}
%    \caption{DPCA-ECDH-PSI}
% \end{figure*}

\input{protocols/revised_protocol.tex}

==> sections_bak/3_dp.tex <==
%!TEX root = ../main.tex
\section{Two-Party Dual-Sided DP for PSI }\label{sec:dp}
\jd{In the literature, DP is commonly categorized into two models: the central model and the local model.
In the central model of DP, each user submits their data to an aggregator without any added noise. The aggregator then processes this data using a DP mechanism.
On the other hand, in the local model of DP, while there still exists an aggregator, they do not have access to the real data. Instead, each user applies a DP mechanism to their own data locally. Only after anonymizing their data do they transmit it to the aggregator. 
However, the PSI protocol is a distributed computation without an aggregator.}
Our focus lies in two-party dual-sided DP~\cite{mcgregor2010limits}. Our goal is to enable two parties to collaboratively compute the desired output while ensuring privacy for \emph{both} inputs.
The definition is provided below.
\newpage
\begin{definition}
[Two-party dual-sided $(\epsilon,\delta)$-DP]
A randomized mechanism $\mathcal{M}: \mathcal{A}, \mathcal{B} \rightarrow \mathcal{O}$ provides $(\epsilon, \delta)$-DP for A if for all adjacent inputs\footnote{We focus on the unbounded DP, \ie, two datasets $A$ and  $A'$
 are considered adjacent if 
$A$ can be obtained from 
$A'$ by adding or removing one record represented by multiple IDs.} $A, A' \in \mathcal{A}$ and all subsets $o \subseteq \mathcal{O}$,
\begin{equation}
\label{eq:dp}
\Pr[\mathcal{M}(A, B) \in o] \leq e^\epsilon \Pr[\mathcal{M}(A', B) \in o]+\delta,
\end{equation}
and
same holds for neighboring dataset $B$ and $B'$ given the same $A$.
% \label{def:dp}
\end{definition}
\jd{The standard definition of DP is notably strong, as it ensures privacy even against an adversary with unlimited computational resources. However, many MPC protocols typically assume a computationally bounded adversary. In order to ensure compatibility of the proposed two-party dual-sided DP with PSI and down-stream MPC tasks, we adopt computational DP~\cite{crypto/MironovPRV09}, an analogue of DP that only necessitates privacy against a feasible (i.e., polynomial time) adversary. We provide the corresponding simulation-based computational DP and security analysis later in Section~\ref{sec:dpca-psi}. }


  % We also construct the view of our protocols for the security proof in Appendix~\ref{sec:appendix_dp_proof}.
% We denote the $\view$ of Party A during an execution of $\Pi$ on input sets $A$ and $B$ as $\view^{\Pi}_{P_A}(A,B)$, which is a joint probability distribution over $A$.

% the transcript of the protocol including the revealed intersection size, and private randomness of Party A. For each set $A$, $\view^{\Pi}_{\text{A}}(A,B)$ is a mechanism over $B$. Let $\view^{\Pi}_{\text{B}}(A, B)$ be similarly defined view of Party $B$ whose input is $B$.
  


% \begin{definition}[The view of a protocol execution~\cite{cu/Goldreich2004}]\label{def:view}
% Let $f: \{0,1\}^\ast \times \{0,1\}^\ast \rightarrow \{0,1\}^\ast \times \{0,1\}^\ast$ be a functionality, and $f_{P_A}(A,B)$ (resp., $f_{P_B}(A,B)$) denote the first (resp., second) element of $f(A,B)$. 
% Let $\Pi$ be a two-party protocol for computing the function $f$.
% The $\view$ of the first (resp., second) party during an execution of $\Pi$ on $(A,B)$, denoted $\view^{\Pi}_{P_A}(A,B)$ (resp.,$\view^{\Pi}_{P_B}(A,B))$), is $(A, r, m_1, \ldots, m_t)$ (resp., $(B, r, m_1, \ldots, m_t)$), where $r$ represents the output of the first (resp., second) party's internal coin tosses, and $m_i$ represents the $i$-th message it has received. 
% \end{definition}
% We will show our proposed DPCA-PSI obtain intersection size under the two-party distributed DP following the definition below.
% \begin{definition}
% [DP for two-party PSI protocols] A protocol $\Pi$ is $(\epsilon, \delta)$-differential privacy if the mechanism $\view^{\Pi}_{P_A}(A,B)$ is $(\epsilon, \delta)$-differential privacy for  $B$ and same holds for $\view^{\Pi}_{P_B}(A, B)$.
% \end{definition}
% The privacy definition above ensures the privacy of both $A$ and $B$ against semi-honest adversary.
% In the following section, we suggest incorporating a specially designed dummy random variable padding method to achieve a two-party differentially private intersection size.

\subsection{Two-Party DP for Single-ID Matching}
\label{sec:single_id_dp}
% Distributed noise generation is implemented in a two-party DP mechanism, with each party contributing their respective sub-noise as input in the PSI protocol. During the execution of the PSI protocol, the cardinality of the PSI is protected under the proposed DP mechanism, where the noise is the random variable of the intersection cardinality introduced from both parties.
\begin{algorithm}[b]
% \footnotesize
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Set $A$ and $B$  in Party A and Party B, separately.}
\Output{$A_\mathsf{up}$  and $B_\mathsf{up}$ for PSI input}

{Generate a common set  $D$ of size $2\tau$ that is disjoint from both $A$ and $B$.}


{Party A obtains $D_A$ by randomly shuffling $D$ and then selecting the first $\tau$ elements.}


{
Party A pads with dummy values to obtain $A_\mathsf{up} = A \cup D_A$.}

{Party B obtains $D_B$ by randomly shuffling  $D$ and then selecting the first $\tau$ elements.}

{
Party A pads with dummy values to obtain $B_\mathsf{up}= B\cup D_B$.}

% {Parties A and B apply $A_\mathsf{up}$ and $B_\mathsf{up}$ as their input individually for any PSI protocol. }
\caption{IntersectMask DP for Single-ID PSI}
\label{alg:DP-SI-SingleID}
\end{algorithm}
We represent the random variable of the intersection size of our proposed DPCA-PSI protocol as $\mathcal{M}(A, B)$. Randomness is introduced by padding dummy entries to both input sets $A$ and $B$ to create $A_\mathsf{up}$ and $B_\mathsf{up}$, respectively. This is done by randomly selecting\footnote{{ We introduce the  the sampling steps in our illustrative example in~\Cref{sec:example}. }} and adding $\tau$ dummy entries from a common set $D$ with $2\tau$ rows, which is disjoint from both $A$ and $B$.
The specific steps are outlined in Algorithm~\ref{alg:DP-SI-SingleID}.
% Note that, up to this point, $\mathcal{M}(A, B)$ is independent of the PSI procedure.
The following lemma demonstrates the Probability Mass Function (PMF) of the randomness introduced to the intersection size. 
\begin{lemma}
\label{lemma:set_cdn_pmf} 
The size of the intersection between two padded sets in Algorithm~\ref{alg:DP-SI-SingleID}, denoted as $|A_\mathsf{up} \cap B_\mathsf{up}|$, can be represented as
\begin{equation}
\label{eq:dpca}
\mathcal M(A, B) \triangleq |A_\mathsf{up}\cap B_\mathsf{up}|
=
|A\cap B| + \mathsf z,
\end{equation}
where $\mathsf z = |D_A\cap D_B|$ with axisymmetrially  PMF:
\begin{equation}
\label{eq:z_dpca}
\P(\mathsf z = z)= \begin{cases}
\frac{(\C_{\tau}^z)^2}{\C_{2\tau}^\tau},\quad &0<z\leq \tau, \\
0,\quad & \text{others}.
\end{cases} 
\end{equation}
\end{lemma}
The proof is postponed to the Appendix~\ref{app:pmf}.
Lemma~\ref{lemma:set_cdn_pmf} shows that via separately padding dummy entries, Algorithm~\ref{alg:DP-SI-SingleID} introduces 
 additive noise to $|A\cap B|$.
In cases where we concentrate on the DP protection of $A$, the inclusion of $B$ is omitted from $\mathcal M(A, B)$ for simplicity (\ie, only $\mathcal{M}(A)$).
Next, we introduce the privacy loss random variable~\cite{dwork2016concentrated} for a tight DP analysis. 

% In our exploration, we will primarily adopt the notations introduced in~\cite{koskela2020tight, meiser2018tight}, from which the majority of the results we utilize are derived.
\begin{definition} 
\label{def:pld}
The privacy loss random variable of $\mathcal M(A)$ over $\mathcal M(A^\prime)$ for any pair of neighboring inputs $A\sim A^\prime$ is defined as follows:

\noindent (i) If both $\P(\mathcal{M}(A)=o)\neq 0$ and $\P(\mathcal{M}(A^{\prime})=o)\neq 0$, then
\begin{equation}
\label{eq:PLD}
\bm \gamma_{AA^\prime} \trian

\ln\left(\frac{\P(\mathcal{M}(A)=o)}{\P(\mathcal{M}(A')=o)}\right).
\end{equation}
(ii) If  $\P(\mathcal{M}(A^{\prime})=o) = 0$ and $\P(\mathcal{M}(A^{\prime})=o) \neq 0$, then
\begin{equation}
\label{eq:PLD_infty}
\bm \gamma_{AA^\prime} \triangleq
\infty.
\end{equation}
\end{definition}
The quantity $\bm \gamma_{AA^\prime}$  
is the logarithmic ratio between the probability of observing outcome $o$ on input $A, B$ compared to input $A', B$, which is referred to as the privacy loss variable. From Definition~\ref{def:pld}, it is apparent that the privacy analysis involves both $\bm \gamma_{AA'}$ and $\bm \gamma_{A' A}$  by considering the order of $A$ and $A^\prime$.
According to %the DP definition in 
Eqn.~(\ref{eq:dp}), $\mathcal M$ assures tightly $(\epsilon,\delta)$-DP with $\delta$ computed as follows:
\begin{equation}\label{eq:6}
\delta_{AA^{\prime}}(\epsilon) \triangleq\! \sum_{o \in O} \max \left(\P(\mathcal M(A)=o)-e^{\epsilon} \P(\mathcal M(A^\prime)=o), 0\right),
\end{equation}
\begin{equation}\label{eq:7}
\delta_{A^{\prime}A}(\epsilon)  \triangleq \!\sum_{o \in O} \max \left(\P(\mathcal M(A^\prime)=o)-e^{\epsilon} \P(\mathcal M(A)=o), 0\right),
\end{equation}
\begin{equation}\label{eq:generaldelta}
\delta(\epsilon)=\max \left(\delta_{AA^{\prime}}(\epsilon), \delta_{A^{\prime}A}(\epsilon)\right).
\end{equation}
To streamline the analysis, we demonstrate the property that when employing a  DP mechanism with axisymmetrially distributed additive noise such as that proposed in Algorithm~\ref{alg:DP-SI-SingleID}, the order of neighboring data sets can be disregarded in the privacy analysis. The proof is provided in Appendix~\ref{app:one-delta}.
\begin{property}\label{prop:sym}
\label{prop:symmetric}
If and only if the PMF of $\mathcal{M}(A)$ is axisymmetrically distributed, as exemplified by $\P(\mathsf z)$ in Eqn.~(\ref{eq:z_dpca}), the following relationship holds for any non-negative $\epsilon$:
\begin{equation}
\delta_{A^\prime A}(\epsilon)=\delta_{AA^\prime}(\epsilon).
\end{equation}


\end{property}
%  By defining the following quantities:
% \begin{equation}
% \delta(+\infty)\triangleq \P(\bm\gamma=+\infty), \quad  
% \delta(\bm\gamma)\triangleq (1-e^{\epsilon-\gamma})\P(\gamma),
% \end{equation}
Property~\ref{prop:symmetric}  simplifies the DP analysis by allowing the privacy accountant with either \eqref{eq:6} or \eqref{eq:7}. Therefore,  simplify $\bm \gamma_{AA'}$ as $\bm \gamma$. Substituting Eqn.~(\ref{eq:z_dpca}) into Eqn.~(\ref{eq:PLD}), we have
\begin{equation}
\label{eq:PLD1}
    \P_{\bm \gamma}(\bm \gamma = \ln(\C^{z}_{\tau}/\C^{z+1}_{\tau})) = \frac{(\C_{\tau}^z)^2}{\C_{2\tau}^{\tau}}, \quad \forall z\in[0,...,\tau].
\end{equation}
Meanwhile, Eqn.~\eqref{eq:6} can be reformulated as
\begin{equation}
\label{eq:dp_profile}
\begin{aligned}
\delta(\epsilon) & \geq \mathbb{E}_{\bm \gamma}[\max \{0,1-\exp (\epsilon-\gamma)\}] \\
& =\delta(+\infty)+\int_\epsilon^{\infty}(1-\exp (\epsilon-\gamma)) \P_{\bm \gamma}(\gamma) d \gamma.
\end{aligned}
\end{equation}
% The above DP profile can be written
%  as the sum of two expressions as
% \begin{equation}
% \delta(\epsilon) \triangleq \delta(+\infty) + \delta(\bm\gamma>\epsilon).
% \end{equation} 
In this context, $\delta(+\infty)$ addresses failures resulting from the support discrepancy between $\mathcal{M}(A)$ and $\mathcal{M}(A^\prime)$, where a single occurrence leads to infinite leakage, \ie,
\begin{equation}
\label{eq:inf_delta}
\delta(+\infty)=\P(\mathcal{M}(A)=|A\cap B|).
\end{equation}   
By further substituting Eqn.~(\ref{eq:inf_delta}) into the second term in the r.h.s of Eqn.~(\ref{eq:dp_profile}), we acquire the intersection size's Differential Privacy (DP) profile using Algorithm~\ref{alg:DP-SI-SingleID}, as outlined in Theorem~\ref{two_way_dp} below.
 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.35\textwidth]{images/multiid.pdf}
%     \caption{Illustration of the two-party differentially private cardinality release by subsampling in the multi-id setting.}
%     \label{fig:multi-id}
% \end{figure}

\begin{theorem}\label{two_way_dp}
The two-party DP mechanism described in Algorithm~\ref{alg:DP-SI-SingleID}, padding $\tau$ randomly selected dummy entries at each party as PSI input, achieves the output $|A_\mathsf{up} \cap B_\mathsf{up}|$ to be tight $(\epsilon,\delta(\epsilon))$-DP for both parties $A$ and $B$. The profile of $(\epsilon,\delta(\epsilon))$  is given as follows:
\begin{equation}
\label{eq:delta}
    \delta(\epsilon) = \frac{1}{\C_{2\tau}^\tau}
    \left(1 +\sum_{z=\left\lceil\frac{e^{\epsilon/2}\tau-1}{{e^{\epsilon/2}+1}}\right\rceil}^{\tau-1}(\C_\tau^z)^2-e^{\epsilon}(\C_\tau^{z+1})^2\right).
\end{equation}
\end{theorem}
For a given target $(\epsilon, \delta)$, one can calculate the parameter $\tau$ using the DP profile above, which serves as an input to Algorithm~\ref{alg:DP-SI-SingleID}.
\subsection{Two-Party DP for Multi-ID Matching}
% \donghang{this description is duplicated with the Introduction section}
% While PSI protocols have received considerable attention, with notable advancements in efficiency, there exists a notable gap in the exploration of multi-ID matching within the PSI literature. This is in stark contrast to real-world applications where records are typically indexed by various IDs (e.g., phone number, email address, IP address) due to the rarity of parties sharing a single identifier for each user. Performing an exact equality check based on a single ID column when matching records from different entities may lead to a significant number of missed records. In practical scenarios, the need for multi-ID PSI is frequent, yet this aspect remains relatively unexplored in academic research. A commonly employed multi-ID matching logic is the \emph{waterfall-matching}, a ranked deterministic matching logic.
% In this section, we focus on the distributed two-party DP mechanism design for multi-ID matching and defer the corresponding PSI protocol for the multi-ID matching in Section~\ref{sec:dpca-psi}.

DP protection in multi-ID scenarios can be accomplished by applying the single-ID DP mechanism to each ID column. However, given that a single record is represented by multiple IDs, combining the matching results of multiple IDs results in privacy loss, as formalized in the research of DP composition~\cite{dwork2016concentrated}. It is well-known that the composition of DP mechanisms compromises the privacy of DP protection.
Suppose Algorithm~\ref{alg:DP-SI-SingleID} for the $\ell$-ID achieves $(\epsilon_\ell,\delta_\ell)$-DP for its intersection size. The basic composition reveals that DP protection, considering the observation of each intersection size of each ID column from the two parties, is 
$
\left(\epsilon, \delta\right)$-DP, where 
\begin{equation}
\label{eq:basic}
\epsilon=\sum_{\ell=1}^L\epsilon_\ell \quad  \text{and} \quad \delta=\sum_{\ell=1}^L \delta_\ell.
\end{equation}
Consequently, the protective capacity of DP diminishes linearly with an increase in the number of IDs.

The linear rate of diminishing DP is attributed to the fact that different IDs matched for each column could correspond to the same record. For instance, dummy ID1 and dummy ID2 that are matched could both correspond to the same data record, say Alice.
If there is a way to ensure that the cross-ID dummies cover disjoint subsets of the data records, the sequential composition is no longer a tight DP analysis. Instead, the combined privacy loss is the maximum of $\epsilon_\ell$ for all $\ell\in [1, L]$ from the parallel composition theorem.
To ensure that cross-ID dummies cover disjoint subsets of the dummy records, we propose  Algorithm~\ref{alg:DP-multi-ID} to construct dummy variables. The sufficient condition for parallel composition is that the dummies padded for different ID columns come from disjoint spaces and cannot match.
\begin{algorithm}[t]
% \footnotesize
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{The sets $A$ and $B$ in Party A and Party B, respectively, index each data record via $L$ different kinds of IDs.}
\Output{$A_\mathsf{up}$ and $B_\mathsf{up}$}

{Generate $L$  set  $\{D_\ell\}_{\ell=1}^{L}$ each  with size $2\tau$ and being disjoint from both $A$ and $B$.}

{Generate dummy set $D^{\prime}$ with size at least $2\tau(L-1)L$ being disjoint from both $A$ and $B$.}

{\textbf{For} $1 \le \ell \le L$:}

{\quad Party A obtains $D_{A,\ell}$ by randomly shuffling $D_\ell$ and then selecting the first $\tau$ elements from each $D_\ell$.}

{\quad 
Party $A$ pads the $\ell$-th ID column with dummy values $D_{A,\ell}$ to update $A_\mathsf{up}$.}

{\quad Party $A$ randomly selects $\tau(L-1)$ samples from $D^{\prime}$ without replacement and pads selected samples to other $L-1$ ID columns to update $A_\mathsf{up}$. }

{\quad Repeat Step~4-Step~6 for Party B to update $B_\mathsf{up}$ and $D^{\prime}$.}
% {\quad Party B obtains $D_{B,\ell}$ by randomly shuffling $D_\ell$ and then selecting the first $\tau$ elements from $D_\ell$.}

% {\quad 
% Party $B$ pads the $\ell$-th id column with dummy values $D_{B,\ell}$ to update $B_\mathsf{up}$.}

% {\quad Party $B$ randomly selects $\tau(L-1)$ samples from $D^{\prime}$ without replacement, and pads selected samples to other $(L-1)$ id columns to update $B_\mathsf{up}$. $D^{\prime}$ is updated by removing selected samples.}

% {
% Party A pads with dummy values to obtain $B_\mathsf{up}= B\cup D_B$.}
{\textbf{End For}}
% {Parties A and B apply $A_\mathsf{up}$ and $B_\mathsf{up}$ as their input individually for any PSI protocol. }
\caption{IntersectMask DP for Multi-ID PSI}
\label{alg:DP-multi-ID}
\end{algorithm}



 \begin{property}
In Algorithm~\ref{alg:DP-multi-ID}, if padding dummy variables for the $\ell$-th column leads to achieving $(\epsilon, \delta)$-DP for the $\ell$-th column intersection size, then $|A_\mathsf{up} \cap B_\mathsf{up}|$ also achieves $(\epsilon, \delta(\epsilon))$-DP for any multi-ID PSI. The profile of $(\epsilon, \delta(\epsilon))$ is provided in Eqn.~(\ref{eq:delta}).
\end{property}



\subsection{Multi PSI Executions Amplify Privacy Leaks}
Ensuring the practical utility of any PSI involves enabling its execution multiple times on a single dataset or on multiple datasets that share a common individual data record. For example, deploying the PSI service for online ad measurement also requires multiple executions~\cite{Guo2022birds}.

From the privacy perspective, the notion of combining multiple DP intersection results while preserving the overall privacy guarantee is referred to as the sequential DP composition problem. 
One widely adopted analysis is the basic composition shown in Eqn.~(\ref{eq:basic}), revealing a linear increasing rate of $\epsilon$. Given the inversely proportional relationship between the dummy size $\tau$ and $\epsilon$, it is natural to explore a tight DP composition that decreases $\tau$ under the same $\epsilon$.
We adapt the composition results shown in 
\cite{koskela2020tight} to our multiple PSI execution cases.
Given $\P_{\bm \gamma}$ in Eqn~(\ref{eq:PLD1}), 
after $k$ times of execution of
DPCA-PSI, the composition is tightly $(\epsilon, \delta)$-DP for $\delta^k(\epsilon)$ given by
\begin{equation}\label{eq:delta^k}
\begin{aligned}
\delta^k(\epsilon) & =1-\left(1-\delta(+\infty)\right)^k+ 
\int_{\epsilon}^{\infty}\left(1-\mathrm{e}^{\epsilon-\gamma}\right)\left(\P_{\bm \gamma} *^k \P_{\bm \gamma}\right)(\gamma) \mathrm{d} \gamma,
\end{aligned}
\end{equation}
where $\delta^K(\epsilon)$ denotes the post-composition privacy profile, and $\ast^K$ denotes the $K$ times convolution.
According to
Eqn.~(\ref{eq:inf_delta}), it is straightforward that,

% \begin{property}

% Consider a non-adaptive $K$-fold composition of the of two-way DP mechanism in Algorithm~\ref{alg:DP-SI-SingleID}. The composition is tightly $(\epsilon,\delta(\epsilon, K))$-DP  with $\delta(\epsilon)$ being determined by \bj{define $\delta(\epsilon, K)$}
% The 
\begin{equation}\label{eq: k-fold}
% \label{eq: delta_comp}
\begin{aligned}
    \delta^k(\epsilon) &= 1- \left(1-\frac{1}{\C_{2\tau}^\tau}\right)^k
    + \sum_{\gamma:\epsilon<\gamma<\infty}(1-e^{\epsilon-\gamma})\P_{\bm \gamma}(\gamma)^{\circledast k},\\
\end{aligned}
\end{equation}
where $.^{\circledast k} $ denotes the $k$-fold convolution. 
Note that directly solving $\P_{\bm \gamma}(\gamma)^{\circledast k} $ exhibits exponentially computation complexity w.r.t. $k$. Following similar steps as presented in \cite{koskela2020tight}, we present the two-party DP composition accounting algorithm based on FFT in Algorithm~\ref{alg:fft}, subsequently, we outline steps to numerically derive $\tau$ that guarantees $(\epsilon,\delta)$-DP after $k$-fold composition in Algorithm~\ref{alg:bisection}.

FFT-based composition for privacy loss involves representing the distribution as a sparse vector, marking specific locations indicating data leakage and their probabilities. This vector is transformed into the frequency domain using FFT, followed by multiplication operations to handle convolution. Matrix expressions simplify these complex operations into linear transformations and power computations. The processed sequence is then reverted to the time domain using the inverse FFT transformation.

FFT significantly improves the computation cost  from $\mathcal{O}(n^2)$ to $\mathcal{O}(n\log(n))$, where $n$ denotes the length of $\P_{\bm \gamma}(\gamma)^{\circledast k}  $. However, FFT requires the input sequence to be periodic. Further, the input sequence should be cast to a periodical window with size, say $W$, no less than the length of FFT result to avoid information loss due to spectrum overlap. To this end, we proved the following property with details in Appendix~\ref{app:window_len} and it is used to set the parameter $W$ required in DPCA-PSI.

% precisionly compute k-composition is $\mathcal O()$.
% -->FFT -->FFT needs periodic. window larger than ?? to avoid specturem alias. $\mathcal O(\tau)$

\begin{property}
\label{prop: window}
The minimal window size for FFT to guarantee no spectrum overlap is
   \begin{equation}
     W \ge (4K-2)\ln(\tau). \end{equation}
\end{property}


Further, casting continuously-valued leakages to discrete vector locations incurs information loss. The discretization is handled by the resolution factor $n_x$ that represents the total number of entries on the input sequence vector. Intuitively, larger $n_x$ leads to high input resolution, and thereby reduces information loss. However, large $n_x$ inevitably increases the computation complexity. 
By
examining line 4 of Algorithm 3. This line projects the continuously valued leakage onto the closest discretized location to its right. In essence, this means that the leakage is consistently amplified or increased, thereby ensuring that the calculated $\delta$ is always greater than or equal to the true $\delta$ that accurately reflects the exact leakage. Therefore, we have the following conclusion.
% To this end, we next show that the discretization in Algorithm 3 is only over estimating the privacy leakage, i.e., the $\delta$ accounted by Algorithm 3 features the leakage upperbound. 
\begin{property}\label{prop:comp}
The DP parameter $\delta$, computed by Algorithm~\ref{alg:fft}, consistently exceeds or equals the true $\delta$ value that accurately represents the actual data leakage.
\end{property}

\begin{algorithm}[t]
\footnotesize
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Dummy size $\tau$;
 $k$: compositions \#; 
$\epsilon$: target $\epsilon$ after $k$-fold composition;
$W$: FFT periodic window size;
$n_x$: Input sequence density.}


\Output{DP parameter $\delta$ post-composition}

{Compute FFT resolution: $\Delta_x = 2W/n_x$.}

{Initialize PLD vector as an all zeros vector $P_{\Gamma}\in \mathbb R^{n_x}$}

{\text{For} $o\in [0,...,\tau-1]$:}

{\quad Update:  $
    P_{\Gamma}\left[\lceil (W + 2\ln{\C_\tau^o}-2\ln{\C_{\tau}^{o+1}})/\Delta_x\rceil\right]={(\C_\tau^o)^2}/{\C_{2\tau}^\tau} \nonumber
$}

{EndFor}

{Compute the convolutions via FFT: $
 b = D\mathcal{F}^{-1}\left(\mathcal{F}(D\cdot P_{\Gamma})^{K}\right)
,$ where
$D \triangleq \begin{bmatrix}
0 & I_{n_x/2} \\
I_{n_x/2} & 0 
\end{bmatrix}$.\\
}

 {Compute the starting point:
$\gamma_{\epsilon}=\left\lceil\frac{\epsilon+W}{\Delta_x}\right\rceil. \nonumber
$}

{Estimate $\delta$:
$
    \delta = 1- \left(1-\frac{1}{\C_{2\tau}^\tau}\right)^K + \sum_{\gamma=\gamma_{\epsilon}}^{n_x}(1-e^{\epsilon+W-\gamma\Delta_x})b[\gamma]\nonumber.
$} 

\caption{IntersectMask DP DP Composition  }
\label{alg:fft}
\end{algorithm}

\begin{algorithm}[t]
\footnotesize
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Total DP budget $(\epsilon, \delta)$;\\
Total \# of composition: $k$;\\
Any $\tau_{\mathsf{up}}$ that guarantees the corresponding $\delta_{\mathsf{up}}$ computed by Algorithm 3 is less than $\delta$; $\tau_{\mathsf{low}}=0.$}

\Output{\# of dummy added for DP: $\tau$.}

{\text{While} $\tau_{\mathsf{low}}<\tau_{\mathsf{up}}$:}

{\quad Compute $\tau^{\prime} = \frac{1}{2}\lceil\tau_{\mathsf{low}}+\tau_{\mathsf{up}}\rceil$,}

{\quad Compute $\delta^{\prime}(\epsilon, \tau^\prime)$ via Algorithm~\ref{alg:fft}.}

{\quad\text{If} $\delta^{\prime}\geq \delta$:}

 {\quad\quad Compute: $\tau_{\mathsf{low}} = \tau^{\prime}$;}

{\quad\text{Else:}} 

 {\quad\quad Compute: $\tau_{\mathsf{up}} = \tau^{\prime}$;}

{Return: $\tau = \tau_{\mathsf{up}}$.}

\caption{Minimal $\tau$ achieving $(\epsilon,\delta)$-DP}
\label{alg:bisection}
\end{algorithm}
In summary, for a given target $(\epsilon, \delta)$, one can calculate the parameter $\tau$ using via  Algorithm~\ref{alg:bisection}.
Until now, we can compare our FFT-based tight composition method with the basic composition using the same privacy parameters. Consider the settings that $\epsilon = 2$ and $\delta = \frac{1}{10m}$, where $m$ represents the number of data records. The maximum PSI execution number is 18.
Figure~\ref{fig:tau_comp} demonstrates that our FFT-based composition requires a significantly smaller $\tau$, indicating lower communication and computation costs compared to the original PSI protocol, due to the introduced DP protection.

\begin{figure}
    \centering
\includegraphics[width=0.28\textwidth]{images/compo_compare1.pdf}
    \caption{Comparing the  dummy size ($\tau$) between the basic composition and our method for various input sizes. 
    % to achieve $(\epsilon,\delta)$-DP post-composition, with $\tau$ accounted by FFT based algorithm in Algorithm 4, and basic composition, respectively. $\epsilon = 2$, $T = 6$.
    }
    \label{fig:tau_comp}
    \vspace{-0.5cm}
\end{figure}

% \begin{algorithm*}
% \caption{Fourier Accountant Algorithm for Discrete-Valued Mechanisms}\label{alg:cap1}
% \hspace*{\algorithmicindent} \textbf{Input:}\\  $\tau$, $W$: the size of the periodic window  for FFT, e.g. $W=600$; $K$: number of compositions, $\epsilon$: target $\epsilon$ after $K$-fold composition, $nx$: density of the FFT, e.g., $n_x = 10^6$. \\
%  \hspace*{\algorithmicindent} \textbf{Output:} 
%  $\delta$, such that $\mathcal{M}$ is tightly $(\epsilon,\delta)$-DP\\
% Compute FFT resolution: $\Delta_x = 2W/n_x$; Initial PLD as all zeros vector $P_{\Gamma}\in \mathbb R^{n_x}$ ;\\
% Update $P_{\Gamma}$, for all $o\in [1,...,\tau-1]$:
% \begin{equation}
%     P_{\Gamma}\left[\lceil W + 2\ln{\C_\tau^o}-2\ln{\C_{\tau}^{o+1}})/\Delta_x\rceil\right]={(\C_\tau^o)^2}/{\C_{2\tau}^\tau}
% \end{equation}
% Evaluate the convolutions using FFT:
% \begin{equation}
%     b = D\mathcal{F}^{-1}\left(\mathcal{F}(D\cdot P_{\Gamma})^{K}\right),
% \end{equation}
% where $D \triangleq \begin{bmatrix}
% 0 & I_{n_x/2} \\
% I_{n_x/2} & 0 
% \end{bmatrix}$.\\
% Determine the starting point of the integral interval:
% \begin{equation}
%     \gamma_{\epsilon}=\left\lceil\frac{\epsilon+W}{\Delta_x}\right\rceil,
% \end{equation}\\
% Estimate $\delta$ as follows:
% \begin{equation}
%     \delta(\epsilon) = 1- \left(1-\frac{\tau^2}{\C_{2\tau}^\tau}\right)^T + \sum_{\gamma=\gamma_{\epsilon}}^{n_x}(1-e^{\epsilon+W-\gamma\Delta_x})b[\gamma]
% \end{equation}
% \end{algorithm*}









==> sections_bak/3_technical_preliminaries.tex <==
%!TEX root = ../main.tex
% \section{Preliminary}\label{sec:prelim}
% %We describe important notations and definitions used in this paper.  \\
% \textbf{Notations.}
% $\Delta(\cdot, \cdot)$ is the function computing the symmetric difference of two sets. $|\cdot|$ denotes the size when the argument is a set. 
% We say that two databases $D$ and $D'$ are~\emph{adjacent} if their symmetric difference contains at most one record (\ie, $|D\Delta D'| \leq 1$). \bj{$|\Delta(D, D')|$ ?} 
% Let $\mathbf{a} = (\mathbf{a}[1], \ldots, \mathbf{a}[n]) \in \GG^n$ \bj{Define $\GG^n$ ?} be an $n$-dimensional vector and $(\mathbf{a})^\alpha$ be the shorthand of $((\mathbf{a}[1])^\alpha, \ldots, (\mathbf{a}[n])^\alpha)$. 
% Let $\pi: [n] \rightarrow [n]$ be a permutation and $\pi^{-1}:$ %[n] \rightarrow [n]$ 
% be its inverse,~\ie, $\pi^{-1}(\pi(i))=i$ for all $i \in [n]$. 
% We write $\mathbf{a}_\pi$ as the shorthand of the result of applying the permutation $\pi$ on $(\mathbf{a}[1], \ldots, \mathbf{a}[n])$, namely $\mathbf{a}_\pi[\pi(i)] = \mathbf{a}[i]$ for all $i \in [n]$.
% \Cref{tab:notation} summarize the rest of frequently used notations in the paper. 
% %In the subsequent sections, %of this paper, 
% %the following symbols relevant to PSI will also be used:

% \begin{table}
% \caption{Notations}
% \label{tab:notation}
% \centering
% \begin{tabular}{cc}
%   \hline
%   Symbol & Definition \\\hline
%   $m$ & \# of users/rows in Party A \\\hline
%   $n$ & \# of users/rows in Party B \\\hline
%   $(\epsilon,\delta)$ & Total DP budget \\\hline
%   $L$ & \# of PII \\\hline
%   $T$ & Upperbound  of PSI \# allowed \\\hline
%   $D$ & Dummy dataset for providing DP protection\\\hline
%   $S$ & Dummy dataset for filling empty spaces\\\hline
%   $\delta_{t}$ & Dirac delta function centered at $t$\\\hline
%   $W$  & Size of the FFT window\\\hline
%   $\Delta_x$ & FFT resolution\\\hline
% \end{tabular}
% \end{table}

% \subsection{Differential Privacy}
% Let us recall the definitions of differential privacy (DP): 
% \begin{definition}[$\epsilon$-DP privacy]\label{def:edp}
% A randomized mechanism $f: \mathcal{D} \rightarrow \mathcal{R}$ provides $\epsilon$-DP if for all adjacent inputs $D, D' \in \mathcal{D}$ (\ie, $|D \Delta D'| \leq 1$) and all subsets $S \subseteq \mathcal{R}$
% $$
% \Pr[f(D) \in S] \leq e^\epsilon \Pr[f(D') \in S],
% $$
% where the probability space is $f$'s coin tosses. 
% \end{definition}
% A relaxed notion denoted by $(\epsilon, \delta)$-DP has an additional parameter $\delta$. 











==> sections_bak/4_our_protocol.tex <==
\section{DPCA-PSI: Multi-ID PSI Protocol}
\label{sec:dpca-psi}
% disjoin set among different PII col.
In this section, our focus is on the design of multi-ID PSI, given that we have decoupled the DP mechanism from the construction of the PSI protocol. A commonly employed multi-ID matching logic is the \emph{waterfall matching}, a ranked deterministic matching logic as discussed in Section~\ref{sec:intro-multi_id_psi}.
Given the analysis in Section~\ref{sec:intro-multi_id_psi}, which emphasizes that the direct application of existing single-ID PSI is not feasible, and multi-ID PSI is vulnerable to membership attacks due to the exponential growth of the cross-ID intersection size number, we introduce the DPCA-PSI protocol.


% In this section, we focus on the distributed two-party DP mechanism design for multi-ID matching and defer the corresponding PSI protocol for the multi-ID matching in

% In this section, we introduce our DPCA-PSI for securely evaluating multi-ID join from the protocol contr. The protocol consists of two parts: (1) generation of the dummy rows to fulfill the requirements of DP. (2) multi-ID PSI protocol that computes cardinalities of each ID following the waterfall matching logic. The algorithms and the corresponding analysis of the first part are already given in Section~\ref{sec:dp}, so we focus on the second part below. 

% The multi-ID PSI protocol is designed for the semi-honest setting: %where 
% the two parties follow the protocol honestly while trying to extract extra information about the other party's private inputs. The inputs of the protocols are an $m \times L$ matrix for Party A and an $n \times L$ matrix for Party B.

% \subsection{A Strawman Proposal}

% We start with a straw-man proposal and then show how to adapt it to fulfill our requirements. The starting point is to use classic DDH-based PSI protocol for each column and get the cardinality for each column. However, the problem with this construction is that the waterfall matching logic is not applied, namely, one row can lead to intersections in multiple columns. If we build another MPC protocol to check if specific rows are already in the intersection of previous columns, the corresponding cost is significantly larger. 
% Instead, we %decide to 
% process the input sets column by column with single-ID PSI protocols, and we ``delete'' the rows that are in the intersection of the current column, then use the remaining input sets to evaluate the rest of the columns. This process must be done in a private fashion such that no extra information about the intersection set is leaked.


\begin{figure*}[tp] 
    \centering

\fbox{
    \begin{minipage}
    {\textwidth} 
    
    \smallskip
    \textbf{Global Parameters:} 
    \begin{itemize} 
        \item %Computational security parameter $\lambda\in\NN^*$, 
        DDH group $(1^\lambda, \GG, p, g)$, a random oracle $\hash: \bin^*\to\GG$ and differential privacy budget $(\epsilon, \delta)$
    \end{itemize}
    
    \smallskip
    \textbf{Inputs:} 
        The input of party $A$ (resp. party $B$) consists of $m$ (resp. $n$) records. Each record is an $L$-dimensional vector. Each dimension represents an identity key (\eg, name, SSN, address, $\ldots$).
    \begin{itemize}
        \item 
        % Each of the $m$ users in Party A has $L$ different types of PIIs. 
        Party $A$'s input: $\mathsf{PII_A} = [\mathbf{a}_1, \ldots, \mathbf{a}_L]$, where $\mathbf{a}_\ell = (\mathbf{a}_\ell[1], \ldots, \mathbf{a}_\ell[m])^T$ and $\mathbf{a}_\ell[i] \in \{0,1\}^\ast$ for $\ell \in [L], i \in [m]$;  
        
        \item  
         Party $B$'s input: $\mathsf{PII_B} = [\mathbf{b}_1, \ldots, \mathbf{b}_L]$, where $\mathbf{b}_\ell = \left(\mathbf{b}_\ell[1], \ldots, \mathbf{b}_\ell[n] \right)^T$ and $\mathbf{b}_\ell[i] \in \{0,1\}^\ast$ for $\ell \in [L], i \in [n]$. 
    \end{itemize}

    \smallskip 
    
    \textbf{Output:}  Both parties output the same list $(\tilde{c}_1, \ldots, \tilde{c}_L)$, where $\tilde{c}_i$ represents the (noisy) number of matching records found due to the $i$-th identity key. 

        \smallskip  \hrule \smallskip

    \textbf{Setup:} 
    % \begin{itemize}
    %     \item
        Party $A$ and $B$ sample their secret exponents $\alpha = (\alpha_1, \ldots ,\alpha_L)$, $\beta = (\beta_1, \ldots ,\beta_L)$ from $\ZZ_p^L$.  
    % \end{itemize}
    
    \textbf{Protocol:}
    
    \begin{itemize}
        \item \textbf{Step 1: Appending dummy items for differentially private set intersection size:}
        \begin{itemize}
            \item Party $A$ and $B$ add dummy rows to $\mathsf{PII}_\mathsf{A}$ and $\mathsf{PII}_\mathsf{B}$ respectively, by sampling from a shared dummy space for each $\ell\in L$.
            The dummy spaces are independent of each other for different values of $\ell$. Now party $A$'s input $\mathsf{PII}'_\mathsf{A}$ consists of $m'$ records and party $B$'s input $\mathsf{PII}'_\mathsf{B}$ consists of $n'$ records. Refer to Algorithm~\ref{alg:DP-multi-ID} for specifics.
 %{\color{black} Denote the results as $\mathsf{PII'_A} = [\mathbf{a}'_1, \ldots, \mathbf{a}'_L]$ and $\mathsf{PII'_B} = [\mathbf{b}'_1, \ldots, \mathbf{b}'_L]$, where $\mathbf{a}'_\ell = (\mathbf{a}'_\ell[1], \ldots, \mathbf{a}'_\ell[m'])^T$, $\mathbf{b}'_\ell = (\mathbf{b}'_\ell[1], \ldots, \mathbf{b}'_\ell[n'])^T$, for $m' > m$ and $n' > n$. } 
        \end{itemize}

        \item \textbf{Step 2: Column-wise shuffling each record and hashing all the entries. For each column:}
        \begin{itemize}
            \item Party $A$ and $B$ sample a random permutation $\pi_A: [m'] \rightarrow [m']$ and $\pi_B: [n'] \rightarrow [n']$, respectively;
            \item Party $A$ and $B$ apply their own random permutation $\pi_A$ and $\pi_B$ to each~\emph{column} of $\mathsf{PII}_\mathsf{A}$ and $\mathsf{PII}_\mathsf{B}$, respectively. Then, they hash all the entries in the permuted $\mathsf{PII}_\mathsf{A}$ and $\mathsf{PII}_\mathsf{B}$ one-by-one into group elements. Denote the ``\emph{permuted-and-hashed}'' $\mathsf{PII'_A}$ (resp. $\mathsf{PII'_B}$) as $H_A = [h_{\mathbf{a}_1}, \ldots, h_{\mathbf{a}_L}] \in \GG^{m'\times L}$ (resp. $H_B = [h_{\mathbf{b}_1}, \ldots, h_{\mathbf{b}_L}] \in \GG^{n'\times L}$), which should satisfy 
            %such that the entry at the $i$-th row, $j$-th column is 
            $h_{\mathbf{a}_j}[\pi_A(i)] = \hash(\mathbf{a}_j[i])$ (resp. $h_{\mathbf{b}_j}[\pi_B(i)] = \hash(\mathbf{b}_j[i])$).
            
        \end{itemize}
    
        \item \textbf{Step 3: Finding matching records column-by-column in a "waterfall" process via Diffie-Hellman style key exchange}

            \begin{itemize}
                \item  Matching the 1st column as follows: 
                    \begin{enumerate}[label={(\roman*)}]
                        \item Party $A$ (resp. party $B$) raises all the entries in $H_A$ (resp. $H_B$) to the power of $\alpha_1$ (resp. $\beta_1$) and exchanges the result. 
                        Namely, party $A$ receives $H^1_{B2A} = [(h_{\mathbf{b}_1})^{\beta_1}, \ldots, (h_{\mathbf{b}_L})^{\beta_1}]$ and party $B$ receives $H^1_{A 2 B} = [(h_{\mathbf{a}_1})^{\alpha_1}, \ldots, (h_{\mathbf{a}_L})^{\alpha_1}]$;
                            
                        \item Party $A$ raises all the entries in the~\emph{first column} of $H^1_{B2 A}$ to the power of $\alpha_1$ so that they become $(h_{\mathbf{b}_1})^{\alpha_1\beta_1} = ((h_{\mathbf{b}_1}[1])^{\alpha_1\beta_1}, \ldots, (h_{\mathbf{b}_1}[n'])^{\alpha_1\beta_1})^T$. Party $A$ samples a random permutation $\pi_{A_1}: [n'] \rightarrow [n']$, applies it to $(h_{\mathbf{b}_1})^{\alpha_1\beta_1}$ and sends the result $(h_{\mathbf{b}_1})^{\alpha_1\beta_1}_{\pi_{A_1}}$ to party $B$;
                            
                        \item Party $B$ does similarly: it samples a random permutation $\pi_{B_1}$ %: [m] \rightarrow [m]$ 
                        and sends $(h_{\mathbf{a}_1})^{\alpha_1\beta_1}_{\pi_{B_1}}$ to party $A$;
                            
                        \item Party $A$ computes the intersection of $(h_{\mathbf{b}_1})^{\alpha_1\beta_1}$ (computed locally in (ii)) and $(h_{\mathbf{a}_1})^{\alpha_1\beta_1}_{\pi_{B_1}}$ (received from party $B$ in (iii)),~\ie, $h_{\cap, 1} = (h_{\mathbf{b}_1})^{\alpha_1\beta_1} \cap (h_{\mathbf{a}_1})^{\alpha_1\beta_1}_{\pi_{B_1}}$. 
                        Let $\idx_1 = \phi$ be an empty set and $\tilde{c}_1 = |h_{\cap, 1}|$. \\
                        For all $(h_{\mathbf{b}_1}[i])^{\alpha_1\beta_1} \in h_{\cap, 1}$, party $A$ marks the $i$-th row of $H^1_{B2 A}$ as ``deleted'' and adds $i$ to $\idx_1$. Party $A$ further marks the first column of $H^1_{B2A}$ as ``deleted''. Let $H^2_{B2A} = [(h^2_{b2a,2})^{\beta_1}, \ldots, (h^2_{b2a, L})^{\beta_1}] \in \GG^{(n'-\tilde{c}_1)\times(L-1)} $ denote the remaining matrix (after removing the column and rows marked as ``deleted'');

                        \item Party $B$ does similarly as party $A$ in (iv). Let $H^2_{A2 B} = [(h^2_{a2b,2})^{\beta_1}, \ldots, (h^2_{a2b, L})^{\beta_1}] \in \GG^{(m'-\tilde{c}_1)\times(L-1)} $ denote the remaining matrix. %(after removing the column and rows marked as ``deleted''). 
                        \end{enumerate} 


                \item   Matching from the 2nd column to the $L$-th column,~\ie
                for $\ell = 2$ to $L$, both parties perform the following:
                    \begin{enumerate}[label={(\arabic*)}]
                    %\setcounter{enumi}{5}
                        \item Let $H^{\ell}_{B2A}= [(h^\ell_{b2a,\ell})^{\beta_1}, \ldots, (h^\ell_{b2a, L})^{\beta_1}]$ (resp. $H^{\ell}_{A2B} = [(h^\ell_{a2b,\ell})^{\alpha_1}, \ldots, (h^\ell_{a2b, L})^{\alpha_1}]$) denote the remaining matrix at party $A$ (party $B$) after columns and rows removal in the previous matching; 

                        \item Party $A$ raises all the entries in the~\emph{first column} of $H^{\ell}_{B2 A}$ to the power of $\alpha_\ell$ to get  $(h^\ell_{b2a,\ell})^{\alpha_\ell\beta_1}$. Party $A$ applies a random permutation $\pi_{A_\ell}$ to $(h^\ell_{b2a,\ell})^{\alpha_\ell\beta_1}$ and sends the result $(h^\ell_{b2a,\ell})^{\alpha_\ell\beta_1}_{\pi_{A_\ell}}$ to party $B$;
                            
                        \item Party $B$ does similarly: it samples a random permutation $\pi_{B_\ell}$ %: [m] \rightarrow [m]$ 
                        and sends $(h^\ell_{a2b,\ell})^{\alpha_1\beta_\ell}_{\pi_{B_\ell}}$ to party $A$;

                        \item Party $A$ raises all the entries in $(h^\ell_{a2b,\ell})^{\alpha_1\beta_\ell}_{\pi_{B_\ell}}$ to the power of $\alpha_\ell \times \alpha_1^{-1}$ and returns the result $(h^\ell_{a2b,\ell})^{\alpha_\ell\beta_\ell}_{\pi_{B_\ell}}$ to party $B$;

                        \item Party $B$ does similarly and returns $(h^\ell_{b2a,\ell})^{\alpha_\ell\beta_\ell}_{\pi_{A_\ell}}$ to party $A$;

                        \item Party $A$ reverts the permutation $\pi_{A_\ell}$ to get back $(h^\ell_{b2a,\ell})^{\alpha_\ell\beta_\ell}$ and computes the intersection $h_{\cap, \ell} = (h^\ell_{b2a,\ell})^{\alpha_\ell\beta_\ell} \cap (h^\ell_{a2b,\ell})^{\alpha_\ell\beta_\ell}_{\pi_{B_\ell}}$. Let $\idx_\ell = \phi$ be an empty set and $\tilde{c}_\ell = |h_{\cap, \ell}|$.\\ For all elements in $(h^\ell_{b2a,\ell})^{\alpha_\ell\beta_\ell}$ that lie in the intersection $h_{\cap, \ell}$, party $A$ recovers the corresponding index back in $H^1_{B2A}$ and adds the index to $\idx_\ell$. (Recall that $(h^\ell_{b2a,\ell})^{\alpha_\ell\beta_\ell}$ is the result of removing rows and columns from $H^1_{B2A}$.) Party $A$ further marks those rows as ``deleted'' and removes the $\ell$-th column in $H^1_{B2A}$. Let $H^{\ell+1}_{B2A}$ denote the remaining matrix after removal;

                        \item Party $B$ performs similarly as party $A$ above. Let $H^{\ell+1}_{A2B}$ denote the remaining matrix after removal. 
                \end{enumerate}         
            \end{itemize}

      \item \textbf{Step Four: Output}
        \begin{itemize}
            \item Party $A$ and $B$ both output the same $L$ integers $(\tilde{c}_1, \ldots, \tilde{c}_L)$, where $\tilde{c}_\ell = |h_{\cap, \ell}|$ for all $\ell \in [L]$ computed from above.
        \end{itemize}  
    \end{itemize}
    \end{minipage}
}

    \caption{Multi-ID DPCA-PSI and Compute $\Pi_{{\mathsf{DPCA-PSI}}}$}
    \label{Alg:DPSetIntersection-temp'}
\end{figure*}

% \subsection{Our Construction}
\jd{
\textbf{Security model:}
Building upon existing ECDH-PSI protocols~\cite{meadows1986more, ion2020deploying, bhowmick2021apple, meta-password, multi_key_meta}, we assume that the participants are semi-honest, meaning they adhere to the protocol specifications but may attempt to glean additional information through supplementary local computations. For instance, recent studies have proposed membership inference attacks~\cite{Guo2022birds, Bo}. 
The semi-honest security model aligns with practical scenarios where the involved parties are bound by contractual obligations to adhere to computation protocols.
Adopting a stronger security model, e.g., malicious model,  is not the primary focus of this work.
}

We present our protocol denoted as $\Pi_{\mathsf{DPCA-PSI}}$ in Figure~\ref{Alg:DPSetIntersection-temp'}. 
% The corresponding notations are defined below.
% Let $\GG$ be a group where the Decisional Diffie Hellman (DDH) assumption holds.
% Let $\mathbf{a} = (\mathbf{a}[1], \ldots, \mathbf{a}[n]) \in \GG^n$ be an $n$-dimensional vector and $(\mathbf{a})^\alpha$ be the shorthand of $((\mathbf{a}[1])^\alpha, \ldots, (\mathbf{a}[n])^\alpha)$. 
% Let $\pi: [n] \rightarrow [n]$ be a permutation and $\pi^{-1}$ %[n] \rightarrow [n]$ 
% be its inverse,~\ie, $\forall i \in [n], \pi^{-1}(\pi(i))=i$. 
% We write $\mathbf{a}_\pi$ as the shorthand of %the result of 
% applying the permutation $\pi$ on $(\mathbf{a}[1], \ldots, \mathbf{a}[n])$, namely $\forall i \in [n], \mathbf{a}_\pi[\pi(i)] = \mathbf{a}[i]$.
At a high level, $\Pi_{{\mathsf{DPCA-PSI}}}$ extends the classic ECDH-based PSI protocols~\cite{PS3I,multi_key_meta,google-psi} to support waterfall multi-ID matching logic and it operates in a column-by-column fashion. For each column, different ECDH ``keys'' are used by two parties. Parties first mask their private inputs with ECDH keys, exchange masked inputs, double-encrypt the other party's input sets, and then send back double-encrypted sets. Then both parties can count the number of common elements in double-encrypted sets to decide the cardinality. At the end of the per-column operations, both parties exclude the rows in the intersection from the input sets. Consequently, the deleted rows will not be counted multiple times even when the rest of the columns cause more intersections, and this is consistent with the waterfall matching behavior. Note that both parties have no information about what exact rows are in the intersection as all the operations above are on masked values that cannot be reversed. The protocols for the first column and the rest of the columns are a bit different in two ways: (1) the input sets for the first column are complete without any deletion, however, the rest of the columns use only partial input sets. (2) The input sets for the first column are in plaintext, however, the input sets for the rest of the columns are already masked by the first-round DDH key ($\alpha_1$ and $\beta_1$ in the figure). Therefore, we put different protocol descriptions in the figure to illustrate these differences.

Note that the deletion step at the end of each column operation is necessary because it avoids cross-column information leakage. We summarize this as the following property:
\begin{property}
    $\Pi_{\mathsf{DPCA-PSI}}$ guarantees that there is no cross-ID intersection size leakage.
\end{property}
For example, consider a scenario where two data records share the same values on both the first column and the second column. If we don't delete them after the matching of the first column, they will match again on the second column, and the attacker can figure out how many data records share the same first two columns. For $L$ ID columns, there are in total $2^L$ combinations that the attacker can learn in this way, causing exponentially increasing information leakage. However, with the deletion steps, if a data record is matched in a certain ID column, it will not participate in the rest of the protocols, thus the attacker cannot figure out if any elements cause intersection in multiple columns. Besides, we use different ECDH keys for each column, making the double-encryption of each ID column independent. If the same ID values appear in different columns, the double-encryption is different. This ensures that the attacker cannot link any values across IDs. 

==> sections_bak/5_privacy_analysis.tex <==
%!TEX root = ../main.tex

\subsection{DPCA-PSI Cost and Security Analysis}
\label{sec:security_proof}
\noindent\textbf{Cost Analysis:}
Theoretically, the overall computation and communication complexity are both linear in the sizes of both parties' input sets including dummy elements. However, in actual execution, we expect the performance to be better due to the removal of input elements during execution if they are part of the intersection for a specific column. This results in a gradual reduction in the size of input sets after each column evaluation, resulting in less time and communication in subsequent column evaluations. %require less time and communication. 
This observation positions our protocol as a more favorable choice in waterfall matching, where most intersections occur in the first column, which typically represents the primary ID.
%In the following, we provide the security analysis in the semi-honest model.

\noindent\textbf{ Security Analysis:}\label{sec:proof}
% Protocols in the malicious model generally require much heavier tools (cut-and-choose, zero-knowledge proofs) and could be orders of magnitude less efficient than their semi-honest counterparts. 
Because of space constraints, we relocate the comprehensive simulator-based security proof to Appendix~\ref{sec:appendix_proof}. There, we establish that the synergy of DP and PSI in DPCA-PSI achieves $\SIM$-$\cdp$ as defined in \cite{crypto/MironovPRV09}.


% We recall the relevant definitions of differential privacy in the context of secure two-party computation. 
% Let $\lambda$ denote the (computational) security parameter and $1^\lambda$ will be an implicit input to all the algorithms. 
% Let $\negl[\lambda]$ denote the set of functions that are~\emph{negligible},~\ie, they approaches zero asymptotically faster than the reciprocal of any polynomial in $\lambda$. 
% Two sequences of random variables $X = \{X_\lambda\}_{\lambda \in \NN}$ and $Y=\{Y_\lambda\}_{\lambda \in \NN}$ are computationally indistinguishable if for any non-uniform PPT algorithm $\mathcal{A}$ there exists a negligible funtion $\negl[\lambda]$ such that $|\Pr[\mathcal{A}(1^\lambda, X_\lambda)=1] - \Pr[\mathcal{A}(1^\lambda, Y_\lambda)=1]| \leq \negl[\lambda]$ for all $\lambda \in \NN$.

% Beimel~\etal~\cite{crypto/BeimelNO08} considered~\emph{differentially-private} multi-party computation protocols and focused on information-theoretically secure MPC, which fits well with (information-theoretic) DP. 
% Mironov~\etal~\cite{crypto/MironovPRV09} noted that information-theoretically secure two-party computation is impossible for generic functionalities.
% Hence, they extended the notion of differentially private MPC to the computational setting~\cite{crypto/MironovPRV09}. 
% There are two natural ways to define~\emph{computational differential privacy}:~\emph{indistinguishably-based} and~\emph{simulation-based} definition. 
% Mironov~\etal~\cite{crypto/MironovPRV09} studied the relations between these notions. 
% %They tried several natural ways to define~\emph{computational differential privacy}, and studied the relation among those resulting definitions. 
% All their definitions consider $\epsilon$-DP, but looking ahead, our protocols achieve $(\epsilon, \delta)$-DP only. 
% Therefore, we further relax their definitions to cope with $(\epsilon, \delta)$-DP functionalities below. 

% We follow the definition of computational differential privac
% We follow the existing definitions for differentially private secure two-party computation (for set operations)~\cite{crypto/MironovPRV09,eurosp/KacsmarKLNSSBSO20} below. 
%In particular, we choose to adapt the ``Ideal/Real'' style simulation-based definition of $\cdp$ because it is generally considered stronger than the indistinguishability-based one. (See~\cite{crypto/MironovPRV09}[Theorem 1] and \cite{stoc/HaitnerMST22}[Section 1.3 and Remark 3.18]). 
%Another benefit of using a simulation-based definition of $\cdp$ is that the security parameters of DP (\ie, $\epsilon$ and $\delta$) and computation indistinguishability (\ie, $\negl[\lambda]$) are nicely separated, providing a more fine-grained control. 
%In short, the indistinguishably-based notion is more relaxed~\cite{crypto/MironovPRV09,stoc/HaitnerMST22}. 


%%%%%%%%  Old definition of SIM-CDP  %%%%%%%%%

%\begin{definition}[$(\epsilon, \delta)$-$\SIM$-$\cdp$ Privacy]
%We say that a two-party protocol $\Pi$ ensures $(\epsilon, \delta)$-$\SIM$-$\cdp$ for party $A$ (resp. party $B$) if for every computationally efficient adversary $B$ (resp. $A$), there exists an $(\epsilon, \delta)$-DP (per Definition~\ref{def:eddp}) mechanism $\mathcal{F}(\cdot)$ such that for every $(x,y) \in \{0,1\}^\ast \times \{0,1\}^\ast$, the probability ensembles $\view^\Pi_B(x,y)$ (resp., $\view^\Pi_A(x,y)$) and $\mathcal{F}(x)$ (resp., $\mathcal{F}(y)$) are computationally indistinguishable. 
%\end{definition}
% We recall the definitions of computational differential privacy (CDP) and the view of protocol execution. 
% %%%%%%%%%  Let's go with the ``Real/Ideal'' style of definition  %%%%%%%%%%%%%%%

% \begin{definition}[The view of a protocol execution~\cite{cu/Goldreich2004}]\label{def:view}
% Let $f: \{0,1\}^\ast \times \{0,1\}^\ast \rightarrow \{0,1\}^\ast \times \{0,1\}^\ast$ be a functionality, and $f_{P_A}(A,B)$ (resp., $f_{P_B}(A,B)$) denote the first (resp., second) element of $f(A,B)$. 
% Let $\Pi$ be a two-party protocol for computing the function $f$.
% The $\view$ of the first (resp., second) party during execution of $\Pi$ on $(A,B)$, denoted $\view^{\Pi}_{P_A}(A,B)$ (resp.,$\view^{\Pi}_{P_B}(A,B))$), is $(A, r, m_1, \ldots, m_t)$ (resp., $(B, r, m_1, \ldots, m_t)$), where $r$ represents the output of the first (resp., second) party's internal coin tosses, and $m_i$ represents the $i$-th message it has received. 
% \end{definition}

% \begin{definition}[$(\epsilon_\kappa, \delta)$-$\SIM$-$\cdp$ Privacy~\cite{crypto/MironovPRV09,eurosp/KacsmarKLNSSBSO20}]
% \label{def:sim-cdp}
% An interactive protocol ensemble $\{\langle f_\kappa(\cdot),g_\kappa(\cdot)\rangle\}_{\kappa \in \mathbb{N}}$, ensures for $\{f_\kappa\}_{\kappa \in \mathbb{N}}$ $(\epsilon_{\kappa}, \delta)$-$\SIM$-$\cdp$, if for every ensemble $\{g^*_\kappa\}_{\kappa \in \mathbb{N}}$ of efficiently computable randomized interactive functions, there exists an ensemble $\{F_\kappa\}_{\kappa \in \mathbb{N}}$ of $(\epsilon_\kappa, \delta)$-differentially-private mechanisms $F_\kappa(\cdot)$ such that for every $x \in \mathcal{D}$, the probability ensembles $\{VIEW_{\kappa, g^*_\kappa}(x)\}_{\kappa \in \mathbb{N}}$ and $\{F_\kappa(x)\}_{\kappa \in \mathbb{N}}$ are computationally indistinguishable.


% % We say that a two-party protocol $\Pi_{f} : \mathcal{X}^m \times \mathcal{X}^n \rightarrow \mathcal{Z}$ ensures $(\epsilon, \delta)$-$\SIM$-$\cdp$ if there exists an $(\epsilon, \delta)$-DP (per Definition~\ref{def:eddp}) mechanism $\mathcal{\hat{F}}(\cdot, \cdot)$ such that for every input $(x, y) \in \mathcal{X}^m \times \mathcal{X}^n$, the probability ensembles $VIEW{}$

% % the protocol $\Pi_{f}$ is a secure two-party computation protocol for the randomized functionality $\mathcal{\hat{F}}(\cdot, \cdot)$ as per the ``ideal/real''-style definition of secure two party computation~\cite{cu/Goldreich2004}. 
% \end{definition}

% Besides, the security of our protocols relies on the classic Decisional Diffie-Hellman (DDH) assumption:
% \begin{definition}[DDH Assumption]\label{def:ddh}
% Let $\GG$ be a group (parameterized by security parameter $\lambda$) and $g$ be a generator. We say that the~\emph{Decisional Diffie-Hellman (DDH)} assumption holds in group $\GG$ if for every PPT adversary $\mathcal{A}$:
% $$
% |\Pr[\mathcal{A}(g, g^a, g^b, g^{ab}) = 1] - \Pr[\mathcal{A}(g, g^a, g^b, g^c) = 1]| \leq \negl[\lambda],
% $$
% where the probability is taken over $a \leftarrow \ZZ_q$, $b \leftarrow \ZZ_q$, $c \leftarrow \ZZ_q$ and the random coins of $\mathcal{A}$. 
% \end{definition}

% We now prove the security in the semi-honest model, where we assume both parties follow the protocol steps honestly, but may try to extract as much information about the other party's private inputs as possible.
% Due to the page limit, we refer readers to Appendix~\ref{sec:appendix_proof} for the full proof. In this section, we briefly summarize the corresponding theorem and our proof outline below.


% \begin{theorem}[Security of $\Pi_{\mathsf{DPCA-PSI}}$]
% \label{thm:dppsi}
% The two-party protocol $\Pi_{\mathsf{DPCA-PSI}}$ ensures $(\epsilon, \delta)$-$\SIM$-$\cdp$ for both party $A$ and party $B$. 
% \end{theorem}

% Following the definition of SIM-CDP in Definition~\ref{def:sim-cdp}, the proof consists of two parts.
% The first part of the proof shows that $\Pi_{\mathsf{DPCA-PSI}}$ is a secure two-party computation protocol that implements DPCA-PSI functionalities. The correctness of the protocol is straightforward as shown by the protocol description. To prove the privacy, we construct the protocol view (Figure~\ref{fig:view_a_1}) and the corresponding simulator $S$ (Figure~\ref{fig:sim_A_new}), then we illustrate that the distributions produced by them are computationally indistinguishable through a series of hybrid arguments. In general, we show that if the adversary can differentiate the outputs from the simulator and the view, the adversary can leverage it to break the DDH assumption. Besides, as $\Pi_{\mathsf{DPCA-PSI}}$ is a symmetric protocol in the sense that the operations of two parties are the same except the input, we only need to prove SIM-CDP for one of the parties, and the other party's proof is trivial by exchanging the roles of two parties in the proof.

% The second part of the proof shows that $\Pi_{\mathsf{DPCA-PSI}}$ (and consequently, the simulator $S$) is an $(\epsilon, \delta)$-differentially private mechanism. As $\Pi_{\mathsf{DPCA-PSI}}$ correctly implements DPCA-PSI functionalities, this proof is reduced to the differential privacy proof of DPCA-PSI (Theorem~\ref{two_way_dp}). Consequently, as the simulator $S$ can only obtain the outputs of DPCA-PSI, which are $(\epsilon, \delta)$-differentially private, $S$ naturally achieves $(\epsilon, \delta)$ differential privacy as well.

% \begin{figure*}[tp]
% \centering
% \fbox{
%     \begin{minipage}{0.9\textwidth}
%     \textbf{Inputs:} $\mathsf{PII_A}=[\mathbf{a}_1, \ldots, \mathbf{a}_L]$, the noise number of matching record per column $(\hat{c}_1, \ldots, \hat{c}_L)$. 

%     \begin{itemize}
%         \item \textbf{Simulate}~party $A$ and party $B$'s \textbf{Step 1 and 2:} 
%             \begin{itemize}
%                 \item In the protocol, party $B$ does not send any message to party $A$ in these two steps. $\SIM_A$ does not need to simulate party $B$'s action here and only need to perform the same steps as party $A$ honestly according to the protocol.  Hence, we skip the full details.
%             \end{itemize}
%         \item \textbf{Simulate}~party $A$ and party $B$'s \textbf{Step 3:} 
%             \begin{itemize}
%                 \item Simulating the steps of matching the 1st column: 
                
%                 \begin{enumerate}
%                     \item $\SIM_A$ simulates a dummy matrix $\bar{H}_A \in \GG^{m'\times L}$ as follows: for each $i \in [m'], j \in [L]$, samples $g_{ij, A} \leftarrow \GG$ and also samples $(\alpha_1, \ldots, \alpha_L) \leftarrow \ZZ^L_q$; % and compute $(g_{ij, A})^{\alpha_1}$; 
%                     \item $\SIM_A$ constructs a dummy matrix $\bar{H}^1_{B2A} \in \GG^{n'\times L}$ under the following constrains (1) %have the colume-wise intersection-size pattern $(\hat{c}_1, \ldots, \hat{c}_L)$ with $\bar{H}_A$, (\ie, 
%                     the $j$-th column of $\bar{H}^1_{B2A}$ has $\hat{c}_j$ common elements with the $j$-th column of $\bar{H}_A$); (2) each row of $\bar{H}_A$ and $\bar{H}^1_{B2A}$ has at most one common element. This is done as follows: 
%                         \begin{enumerate}
%                             \item For $i \in [n'], j \in [L]$:
%                             \item ~~~Let $\max = \sum^j_{k=1} \hat{c}_k$, $\min = \max - \hat{c}_j+1$;
%                             \item ~~~if $i \in [\min,\max]$, $\bar{H}^1_{B2A}[i,j] = g_{ij, A}$;
%                             \item ~~~else sample $\bar{H}^1_{B2A}[i,j]$ uniformly at random, \ie, $\bar{H}^1_{B2A}[i,j] \leftarrow \GG$. 
%                         \end{enumerate}
%                % \item Raise all elements in $\bar{H}_B$ to the power of $\beta_1$, where $\beta_1$ is sampled uniformly at random from $\ZZ_q$.
%                     \item $\SIM_A$ applies a random permutation $\pi_B: [n'] \rightarrow [n']$ to $\bar{H}^1_{B2A}$ row-wise and uses the result as party $B$'s message $H^1_{B2A}$ in Step 3.(i) of the real protocol execution. 
%                     \item $\SIM_A$ follows the protocol description to perform Step 3.(ii).
%                     \item $\SIM_A$ raises all elements in the first column of $\bar{H}_{A}$ to the power of $\alpha_1$, applies a random permutation and uses the result as party $B$ 's message $(h_{\mathbf{a}_1})^{\alpha_1\beta_1}_{\pi_{B_1}}$ in Step 3.(iii). 
%                     \item $\SIM_A$ follows the protocol description to perform Step 3.(iv).
%                 \end{enumerate}

%                 \item Simulating the steps of matching the rest of the columns:

%                 \begin{enumerate}
%                     \item $\SIM_A$ follows the protocol description to perform Step 3.(1) and (2) honestly. 
                    
%                     \item Let $\bar{H}^\ell_{B2A}$, which has $n'-\sum^{\ell-1}_{i=1} \hat{c}_i$ rows, denote the matrix that simulates $H^\ell_{B2A}$ in the real protocol. Note that $\SIM_A$ knows exactly which entries $\bar{H}^\ell_{B2A}[i',j']$ were set to be equal to $g_{i'j', A}$ and which were chosen uniformly at random. $\SIM_A$ samples a new column vector $\bar{h}^\ell_{b2a,\ell}$ consisting of $n'-\sum^{\ell-1}_{i=1} \hat{c}_i$ uniformly random group elements. 
                    
%                     \item $\SIM_A$ further prepares another dummy set $\bar{h}^\ell_{a2b,\ell}$ which is initially empty. $\SIM_A$ sequentially enumerates each entry in the first column of $\bar{H}^\ell_{B2A}$: if the $i$-th entry was chosen to be equal to some  $g_{i'j', A}$, then adds $\bar{h}^\ell_{b2a,\ell}[i]$ to $\bar{h}^\ell_{a2b,\ell}$. After this step, $\bar{h}^\ell_{a2b,\ell}$ should consist of $\hat{c}_\ell$ elements.
                    
%                     \item $\SIM_A$ inserts independent and uniformly random group elements to $\bar{h}^\ell_{a2b,\ell}$ until it contains $m'-\sum^{\ell-1}_{i=1} \hat{c}_i$ group elements. Now for each element in $\bar{h}^\ell_{a2b,\ell}$, $\SIM_A$ raises it to the power of $\alpha_1 \cdot \alpha^{-1}_{\ell}$. $\SIM_A$ applies a random permutation to the resulting $\bar{h}^\ell_{a2b,\ell}$ and uses it as party $B$'s message $(h^\ell_{a2b,\ell})^{\alpha_1\beta_\ell}_{\pi_{B_\ell}}$ in Step 3.(3) of the protocol. 
                    
%                     \item $\SIM_A$ follows the protocol description honestly to perform Step 3.(4). 
                    
%                     \item $\SIM_A$ samples a uniformly random permutation $\pi_{A_\ell}$ and uses $(\bar{h}^\ell_{b2a,\ell})_{\pi_{A_\ell}}$ as party $B$'s message $(h^\ell_{b2a,\ell})^{\alpha_\ell\beta_\ell}_{\pi_{A_\ell}}$ in Step 3.(5). 

%                     \item  $\SIM_A$ follows the protocol description honestly. 
%                 \end{enumerate}
%             \end{itemize}


% %        \item \textbf{Simulate}~party $A$'s \textbf{Step 3 and 4:} 
% %            \begin{itemize}
% %                \item $\SIM_A$ performs the steps honestly as the protocol specified so we skip the details.
% %            \end{itemize}
% %        \item \textbf{Simulate}~party $B$'s \textbf{Step 3:}
% %            \begin{itemize}
% %                \item $\SIM_A$ simulates party $B$'s message in Step 4.(i) by sending $\bar{H}_B$ computed in Step 2 above. $\SIM_A$ simulates party $B$'s message in Step 4.(iii) by sending $((g_{11, A})^{\alpha_1}, \ldots, (g_{m'1, A})^{\alpha_1})^T$.
% %            \end{itemize}
%         %\item \textbf{Simulate}~$A$'s Step 3
%         %\item \textbf{Simulate}~$B$'s Step 3    
%     \end{itemize}

%     \end{minipage}    
% }
%     \caption{Description of $\SIM_A$ for Theorem~\ref{thm:dppsi}}
%     \label{fig:sim_A}
% \end{figure*}



% \begin{figure*}[tp]
%     \centering

    
% \fbox{
%     \begin{minipage}{0.8\textwidth} 
%     \begin{center}
%         $\fdppsi$
%     \end{center}

%     \textbf{Inputs:} 
%     \begin{itemize}
%     \item Both PII records at A and B have $L$ unique IDs, and all users have the same predefined ID order.
%         \item 
%         % Each of the $m$ users in Party A has $L$ different types of PIIs. 
%         The PII records at A, which include $m$ users and $L$ unique IDs for each user, are denoted by
%  $ \mathsf{PII_A} = \left[\mathbf{a}_1,\ldots, \mathbf{a}_L\right]$ with $\mathbf{a}_{\ell}\in\bin^{*\times m}$ and $\ell\in [L]$.
%  The $i$-th row and $\ell$-th column (i.e.,
%  $\mathbf{a}_{\ell}[i]$
%  represents $i$-th user's $\ell$-th PII). %{\color{blue} and a set of values associated with each user $(v^A_1, \ldots, v^A_m)$. }
%         \item  The PII records at B, which include $n$ users, follow the same ID order in A. The PII records in B are denoted by
%  $\mathsf{PII_B} = \left[\mathbf{b}_1,\ldots, \mathbf{b}_L\right]$, where each $\mathbf{b}_{\ell}\in\bin^{*\times n}$. The $\ell$-th PII of the user  in the $j$-th row is denoted by $\mathbf{b}_{\ell}[j]$. %{\color{blue} and a set of values associated with each user $(v^B_1, \ldots, v^B_n)$}.
%     \end{itemize}
%     \smallskip
    
% %    \textbf{Output:}  
% %    \begin{itemize}
% %    \item $\mathsf{PII}_{\cap,A}$ at A and $\mathsf{PII}_{\cap,B}$ at B such that there exists $\ell\in [L]$ for each row $k$ in both $\mathsf{PII}_{\cap,A}$ and $\mathsf{PII}_{\cap,B}$ with $\mathbf{a}_{\ell}[j]=\mathbf{b}_{\ell}[j]$   
% %    \end{itemize}
% %    \smallskip


% \textbf{Output:} Let $\idx_{\cap} = \phi$ be an intially empty set. 
    
% % \begin{enumerate}
% % \item {\color{red}For each column $\ell\in [L]$, append $\tau\times L$ dummies according to Algorithm~YYY. (DP algorithm TBD) and initialize a count $c_\ell= 0$. }. 
% \begin{itemize}
% \item 
% For each column $\ell \in [L]$, compute  $c_{\ell} = |(\mathbf{a}_{\ell} \cap \mathbf{b}_{\ell}) \setminus \{\mathbf{a}_{\ell}[i]\}_{i \in \idx_{\cap}}|$.  
% Let $\idx_\ell$ denote the set of indices of the items in $\mathbf{a}_{\ell}$ that lies in the intersection $\mathbf{a}_{\ell} \cap \mathbf{b}_{\ell}$, namely  $i \in \idx_\ell$ iff. $\mathbf{a}_{\ell}[i] \in \mathbf{b}_{\ell}$, set $\idx_{\cap} = \idx_{\cap} \cup \idx_\ell$. Output $c_\ell + \mathsf z_\ell$. 
% \end{itemize}

%     % \end{enumerate}
%     \end{minipage}
%     }

%     \caption{$\fdppsi$}
%      \label{func:DPSetIntersection-temp}
% \end{figure*}



==> sections_bak/6_discussion.tex <==
\section{DPCA-PSI with Payloads}
\label{sec:dpca-psi-payloads}
% \subsection{DPCA-PSI with Payloads}
% In various real-world scenarios, there is a need for downstream MPC computations on the intersection set. Take the classic ad conversion scenario as an example. The ad conversion counts when a user sees Party B's advertisement placed by Party A, and later makes purchases in the party B's store. The ad publisher (Party A) knows which users have seen the ad for Party B's products, while the company (Party B) possesses information about those who completed purchases and the corresponding revenue. Ideally, both parties aim to collaboratively address two key questions without disclosing their private data: first, determining how many users both viewed an ad and made a corresponding purchase (which can be addressed by DPCA-PSI) and second, calculating the total amount spent by these users. For the latter problem, downstream computation (such as summation in this case) is required after the PSI evaluation.

We demonstrate that DPCA-PSI can be readily modified to facilitate downstream computation by enabling each party to include payloads along with the IDs. The evaluation results will then consist of the secret shares of the payloads corresponding to the elements in the intersection. To accomplish this, both parties send the HE encrypted payloads along with the ID columns in Step 3.(i) of Figure~\ref{Alg:DPSetIntersection-temp'}. Consequently, each party now owns the other party's payloads encrypted by the other party's public key. Then in Step 3 (iv), Party A identifies the intersection, and meanwhile stores the double-encrypted IDs in the intersection and their corresponding payloads, arranging them in alphabet order\footnote{Sorting the double-encrypted IDs in alphabet order leads to the same payloads orders for both parties.}. The same operations are repeated for the rest of the columns. At the end of the protocol, each party stores the HE payloads of the other party corresponding to the intersection set. The final step involves converting HE ciphers to secret shares, ensuring that both parties possess the secret share form of each other's payloads. The conversion between HE ciphers and secret shares is well-studied, and we omit the details here.
We implement the payload variant of DPCA-PSI as well and report the implementation details and the benchmark %can be found 
in Section~\ref{sec:experiments}. 

\subsection{Comparison with Private-ID} 
Private-ID~\cite{multi_key_meta} represents the state-of-the-art multi-ID PSI protocol, however, the paper does not provide a variant with payloads. We observe that their solution can be extended to support payloads through secret-sharing the payloads for all the rows in the union set at the end of the protocol. For the rows that are in the union set but not in one party's input set, ``dummy'' payloads must be appended\footnote{Alternatively, parties can send another vector of $0/1$ shares indicating the membership.}. As a result, the input size of the downstream MPC operations becomes the size of the union set. However, in the context of DPCA-PSI, the input size of the downstream MPC is the size of the intersection. This difference could have a significant impact in many scenarios, especially in unbalanced settings. For instance, in online advertisement conversion cases, the advertiser's database is usually huge (in the billions). Assume only $1\%$ of the users buy products after viewing the advertisement, the intersection set size will be roughly $100$ times smaller than the union set size, which implies that the overhead of the downstream MPC will be $100\times$ cheaper with DPCA-PSI.

Besides, DPCA-PSI also achieves better privacy beyond the DP protection of the cardinality. In Private-ID, the entire database is double-encrypted with the same pair of keys, inadvertently leaking relationships between multiple columns. For example, the attacker can figure out if the same ID appears in multiple columns. Besides, the attack can see if the same row of data triggers more than one intersection. DPCA-PSI inherently addresses and prevents these additional leakages in the protocol design.

==> sections_bak/8_exp.tex <==
\section{Experiments}\label{sec:experiments}

In this section, we present the implementation and benchmark results of the DPCA-PSI protocol. We implement two variants of the DPCA-PSI protocol in C++, one with the HE-encrypted payloads and the other without payloads. \skz{We open-sourced our protocols at [anonymized link]. Our implementation details can be found in Appendix~\ref{app:implementation}.}
\jd{We have demonstrated the robustness of DPCA-PSI against membership inference leakage under state-of-the-art attacks. In the following sections, we compare the efficiency of DPCA-PSI with existing ECDH-PSI protocols.}


% \subsection{The dummy set size with different DP parameters}
% To begin with, we summarize the size of the generated the dummy set given different DP parameters, and we compare our numbers with the basic DP composition. The results are available in Table~\ref{tbl:dp_tau}. \donghang{@Jian: inputs here}

% \begin{table*}[!htbp]  \footnotesize
% 	\caption{Dummy size for DPCA-PSI with 3 columns of IDs. The DP budget is set for a maximum $T = 18$ PSI executions.}  
%  	\centering\setlength{\extrarowheight}{2pt}
% 	\label{tbl:dp_tau}

% 	\begin{tabular}         {>{\centering\arraybackslash}p{1.2cm}|
%        >{\raggedleft\arraybackslash}p{1.5cm}|
%        >{\raggedleft\arraybackslash}p{1.5cm}|
%        >{\raggedleft\arraybackslash}p{1.5cm}|
%        >{\raggedleft\arraybackslash}p{1.5cm}|
%        >{\raggedleft\arraybackslash}p{1.5cm}|
%        >{\raggedleft\arraybackslash}p{1.5cm}
%       }%{c|r|r|r|r|r|r}%{|p{1.2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
% 		\toprule
% 		\multirow{2}*{Input size} &  \multicolumn{2}{c|}{$\epsilon = 2$} &  \multicolumn{2}{c|}{$\epsilon = 4$}&  \multicolumn{2}{c}{$\epsilon = 6$}\\ 
% 		\cline{2-7}
% 		       & Basic DP Composition& Our DP Composition & Basic DP Composition& Our DP Composition &Basic DP Composition& Our DP Composition  \\
%          \hline
%          $10^3 $ &  $6847$ & $433$ & $1910$  & $133$ & $905$ & $68$\\
%          \hline
%          $10^4 $ &  $9301$ & $573$ & $2535$  & $169$ & $1186$ & $84$\\
%          \hline
%          $10^5 $ &  $11857$ & $717$ & $3179$  & $205$ & $1475$ & $101$\\
%          \hline
%          $10^6 $ &  $14513$ & $864$ & $3843$  & $243$ & $1770$ & $118$\\
%          \hline
%          $10^7 $ &  $17023$ & $1014$ & $4515$  & $281$ & $2071$ & $135$\\
%          \bottomrule

% 	\end{tabular}
% \end{table*}

\subsection{Benckmark of Non-payload DPCA-PSI}

Table~\ref{tbl:benchmark_dpca_psi_multicol_no_payload} illustrates the performance of the DPCA-PSI protocol under non-payload multi-ID setting. The input sets are constructed 
in a way that around half of them are in the intersection set according to waterfall logic. Besides, we set the ratio of the intersection distribution among three columns as $85:10:5$, which simulates the real-world scenario where the first column is usually the primary ID thus most of the intersections should happen there. We also simulated three network settings to represent LAN, WAN with good bandwidth, and WAN with bad bandwidth. The benchmark results show that we can achieve the PSI of two sets with the size $10^4$ in around one second with $4$MB communication. 

Note that increasing the PSI execution times will lead to an increase in $\tau$, consequently raising both communication and computation times. However, the incremental effect due to the increase in $\tau$ is negligible, as shown in Fig. 4, because the ratio to the input sizes is small.
% We observe that when the input set is small (\eg, $10^3$), the number of dummy rows that we add for DP is considerably large compared with the original input size. However, as the input size increases, the effects of dummy rows become almost negligible as shown by $\tau$ in the table. Therefore, the running time and communication increase almost linearly with the original input set size. It's worth noting that the communication costs of the experiments in various network settings are marginally different due to the non-deterministic nature of the intersection caused by dummy rows. Given the negligible difference, we only record the communication cost for $10$Gb \& $0.2$ms setting as a baseline in the table. This applies to the rest of the tables as well.


\begin{table}[h]  \footnotesize
	\caption{Benchmark of DPCA-PSI protocol without payloads. The input set of each party has equal size and three ID columns. 
 $\tau$ is the dummy size allowing a maximum of 6 times of PSI executions with $\epsilon = 2$. }  
	\centering\setlength{\extrarowheight}{2pt}
         \label{tbl:benchmark_dpca_psi_multicol_no_payload}

	\begin{tabular} {c|c|r|r|r|r}%{p{1.2cm}|p{1.2cm}|p{2cm}|p{2cm}|p{2cm}|p{2.5cm}}
		\toprule
		\multirow{2}*{\thead{Input\\size}} & \multirow{2}*{$\tau$} & \multicolumn{3}{c|}{Time (sec)} &  \multirow{2}*{\thead{Comm.\\(MB)}}
  \\  \cline{3-5}
		%
		 && $10$Gb \& $0.2$ms & $100$Mb \& $50$ms & $10$Mb \& $50$ms &  \\
         \hline
         $10^3 $ &  $144$ & $0.8$ & $4.5$  & $5.3$ & $1.06$ \\
         \hline
         $10^4 $ &  $191$ & $0.9$ & $5.5$  & $8.1$ & $4.03$ \\
         \hline
         $10^5 $ &  $239$ & $6.0$ & $12.5$  & $37.4$ & $31.83$ \\
         \hline
         $10^6 $ &  $289$ & $49.8$ & $80.7$  & $327.7$ & $307.60$ \\
         \hline
         $10^7 $ &  $340$ & $502.5$ & $770.0$  & $3242.2$ & $3063.02$ \\
         \bottomrule
	\end{tabular}
\end{table}

\noindent\textbf{Comparison with other multi-ID PSI without payloads.}
We obtain the code of Private-ID~\cite{multi_key_meta} protocol from Github and test its performance with the same hardware and network environment. Private-ID is implemented in Rust while our protocol is implemented in C++. \skz{Rust and C++ are comparable regarding overall speed and performance, often with Rust ahead. Therefore,} the impact of the programming language difference should be negligible. The benchmark results can be found in Table~\ref{tbl:benchmark_comparison}.As the input set size increases, our protocol shows significant improvement in both execution time and communication. For instance, we achieve a $25\times$ improvement on running time with the input set size $10^7$. The performance advantage stems from several factors: (1) Our protocols remove elements during execution, resulting in fewer and fewer elements being processed in each round; (2) Our protocol demonstrates greater advantages when the number of IDs is small; (3) Additional contributions to performance come from engineering optimizations.

\begin{table}[h]  \footnotesize
	\caption{Performance comparison between no-payload DPCA-PSI and multi-ID Private-ID protocol~\cite{multi_key_meta}. Each set contains three columns of IDs. Both protocols are executed in LAN setting with $10$Gb bandwidth and $0.2$ms latency. }%$\tau$ represents the  dummy size generated by our DP mechanism.}  
        \centering\setlength{\extrarowheight}{2pt}
	\label{tbl:benchmark_comparison}

	\begin{tabular} {c|r|r|r|r} %{|p{1.2cm}|p{1.2cm}|p{2cm}|p{2cm}|p{2cm}|p{2.5cm}|}
		\toprule
		\multirow{2}*{Input size} & \multicolumn{2}{c|}{Time (sec)} &  \multicolumn{2}{c}{Comm. (MB)} \\ 
		\cline{2-5}
		 & DPCA-PSI & Private-ID & DPCA-PSI & Private-ID \\
         \hline
         $10^3 $ & $0.8$ & $1.4$  & $1.06$ & $0.5$ \\
         \hline
         $10^4 $& $0.9$ & $12.8$  & $4.03$ & $5.1$ \\
         \hline
         $10^5 $ & $6.0$ & $126.2$  & $31.83$ & $49.3$ \\
         \hline
         $10^6 $ & $49.8$ & $1267.7$  & $307.60$ & $475.5$ \\
         \hline
         $10^7 $ & $502.5$ & $12687.8$  & $3063.02$ & $4725.3$ \\
         \bottomrule
	\end{tabular}
\end{table}


\subsection{Benckmark of DPCA-PSI with Payloads}
Table~\ref{tbl:benchmark_with_payload_dpcapsi} illustrates the benchmark of the DPCA-PSI in the multi-ID setting with payloads. DPCA-PSI is the only protocol that supports such scenarios since Private-ID does not support adding payloads and P$\text{S}^3$I does not support multi-ID. Compared with the non-payload variant, the running time increases by around $3\times$, and the communication increases by $5\times$. This is mainly due to the computation and the transfer of the payloads encrypted by Paillier Encryption. We also run experiments on both the balanced and unbalanced input sets, and the results show consistent patterns.

\begin{table*}[!htbp]  \footnotesize
	\centering\setlength{\extrarowheight}{2pt}
	\caption{Performance of DPCA-PSI with payloads. Each party has three columns as IDs and one column of values as payloads. $\tau$ represents the size of the dummy set generated by our DP mechanism. The numbers in the figure represent the running time in seconds (except communication).}  
	\label{tbl:benchmark_with_payload_dpcapsi}

	\begin{tabular}
   {>{\centering\arraybackslash}p{1.2cm}|
   >{\centering\arraybackslash}p{0.6cm}|
   >{\raggedleft\arraybackslash}p{1cm}|
   >{\raggedleft\arraybackslash}p{1cm}|
   >{\raggedleft\arraybackslash}p{1cm}|
   >{\raggedleft\arraybackslash}p{1cm}|
   >{\raggedleft\arraybackslash}p{1cm}|
   >{\raggedleft\arraybackslash}p{1cm}|
   >{\raggedleft\arraybackslash}p{1cm}|
   >{\raggedleft\arraybackslash}p{1cm}
  } %{p{1.2cm}|p{1.2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}}
		\toprule
		\multirow{3}*{Input size} & \multirow{3}*{$\tau$} & \multicolumn{4}{c|}{Balanced} &  \multicolumn{4}{c}{Unbalanced} \\ 
		\cline{3-10}
		 && $10$Gb \& $0.2$ms & $100$Mb \& $50$ms & $10$Mb \& $50$ms & Comm. (MB) &  $10$Gb \& $0.2$ms & $100$Mb \& $50$ms & $10$Mb \& $50$ms & Comm. (MB)  \\
         \hline
         $10^3 $ &  $144$ & $1.1$ & $6.0$  & $10.0$ & $5.68$ & $1.1$ & $5.6$  & $9.0$ & $4.5$ \\
         \hline
         $10^4 $ &  $191$ & $3.3$ & $9.4$  & $27.1$ & $22.72$ & $2.6$ & $7.8$  & $17.9$ & $12.57$ \\
         \hline
         $10^5 $ &  $239$ & $18.5$ & $38.9$  & $186.5$ & $183.56$ & $17.1$ & $28.4$  & $92.4$ & $81.88$\\
         \hline
         $10^6 $ &  $289$ & $176.7$ & $336.1$  & $1771.8$ & $1778.8$ & $160.8$ & $229.8$  & $839.3$ & $763.86$\\
         \hline
         $10^7 $ &  $340$ & $1760.0$ & $3314.1$  & $17616.9$ & $17718.8$ & $1594.1$ & $2250.9$  & $8309.4$ & $7570.89$\\
         \bottomrule
	\end{tabular}
\end{table*}

\noindent\textbf{Comparison with P$\text{S}^3$I with Payloads.}
We also perform the benchmark under the single-ID setting with payloads, and we compare the results with the P$\text{S}^3$I protocol~\cite{PS3I}. Table~\ref{tbl:benchmark_with_payload_single_id} contains the benchmark results with both balanced input sets and unbalanced input sets. In general, the running time of DPCA-PSI is at least $100\times$ faster than P$\text{S}^3$I and the communication is approximately $2\times$ better. This improvement is a result of multiple factors. First, parties in DPCA-PSI only send back HE ciphers that are in the intersection, while P$\text{S}^3$I has to transfer all HE ciphers. Besides, The HE operations supported by the IPCL library in C++ are significantly faster than the Paillier Encryption library in Rust. HE operations are also the main bottleneck of the whole process.

% HE operations are also the main bottleneck of the whole process. What's more, the ECC operations in our protocols are fully accelerated through multi-threading, bringing us a linear factor of performance improvement.


\begin{table*}[!htbp]  \footnotesize
	\centering\setlength{\extrarowheight}{2pt}
	\caption{Performance of single-ID DPCA-PSI with payloads and the comparison with P$\text{S}^3$I~\cite{PS3I} protocol. Each party has one column as ID and one column of values as payloads. $\tau$ represents the size of the dummy set generated by our DP mechanism. The network setting is LAN with $10$Gb bandwidth and $0.2$ms latency. (DP parameters $T = 6, \epsilon = 2$)}  
	\label{tbl:benchmark_with_payload_single_id}

	\begin{tabular}
        {>{\centering\arraybackslash}p{1.2cm}|
       >{\centering\arraybackslash}p{0.6cm}|
       >{\raggedleft\arraybackslash}p{1.3cm}|
       >{\raggedleft\arraybackslash}p{1cm}|
       >{\raggedleft\arraybackslash}p{1.3cm}|
       >{\raggedleft\arraybackslash}p{1cm}|
       >{\raggedleft\arraybackslash}p{1.3cm}|
       >{\raggedleft\arraybackslash}p{1cm}|
       >{\raggedleft\arraybackslash}p{1.3cm}|
       >{\raggedleft\arraybackslash}p{1cm}
      }
 %{p{1.2cm}|p{1.2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}}
		\toprule
		\multirow{3}*{Input size} & \multirow{3}*{$\tau$} & \multicolumn{4}{c|}{Balanced} &  \multicolumn{4}{c}{Unbalanced} \\ 
		\cline{3-10}
		 && \multicolumn{2}{c|}{Time (sec)} & \multicolumn{2}{c|}{Comm. (MB)} & \multicolumn{2}{c|}{Time (sec)} & \multicolumn{2}{c}{Comm. (MB)}\\
		\cline{3-10}
		 && DPCA-PSI & P$\text{S}^3$I & DPCA-PSI & P$\text{S}^3$I & DPCA-PSI & P$\text{S}^3$I & DPCA-PSI & P$\text{S}^3$I  \\
         \hline
         $10^3 $ &  $144$ & $0.6$ & $82.7$  & $1.92$ & $1.9$ & $0.5$ & $50.4$  & $0.96$ & $1.13$ \\
         \hline
         $10^4 $ &  $191$ & $2.0$ & $813.2$  & $15.99$ & $18.6$ & $1.6$ & $462.0$  & $6.43$ & $11.25$ \\
         \hline
         $10^5 $ &  $239$ & $14.8$ & $8183.4$  & $155.69$ & $185.5$ & $12.1$ & $4589.0$  & $60.03$ & $112.2$\\
         \hline
         $10^6 $ &  $289$ & $143.1$ & --  & $1551.40$ & -- & $117.7$ & --  & $594.87$ & --\\
         \hline
         $10^7 $ &  $340$ & $1414.4$ & --  & $15507.60$ & -- & $1168.9$ & --  & $5941.72$ & --\\
         \bottomrule
	\end{tabular}
\end{table*}


\subsection{ Different Intersection Ratios Impact}
% We also explore how the input sets can influence the performance. To begin with, we test both balance sets and unbalanced sets as the inputs. The result is available in Table~\ref{tbl:benchmark_no_payload_balanced}. It can be seen that the performance in the unbalanced setting is better than the balanced setting in both the running time and the communication. This is consistent with the intuition since the size of one of the input sets is significantly smaller, thus reducing the overall communication cost. 

% Besides, w

We adjust the intersection ratio, which is the intersection size divided by the input set size, to see its influence on the performance. Table~\ref{tbl:benchmark_intersection_ratio} shows the benchmark results where we fix the input set size and DP setting, and only change the intersection ratio. It can be seen that the running time decreases as the intersection ratio increases. The underlying reason is that with a higher intersection ratio, more elements will be eliminated during the protocol execution, so the costs of subsequent rounds are reduced. We note that this does not violate our security definition because the intersection ratio can be computed through MPC output directly.


% \begin{table*}[!h]  
% 	\caption{Performance of DPCA-PSI with balanced input sets and unbalanced input sets. Each set contains three columns of IDs with no payload. $\tau$ represents the size of the dummy set generated by our DP mechanism. The network setting is LAN with $10$Gb bandwidth and $0.2$ms latency.}  
%  	\centering
% 	\label{tbl:benchmark_no_payload_balanced}

% 	\begin{tabular}{|p{1.2cm}|p{1.2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
% 		\hline
% 		\multirow{3}*{Input size} & \multirow{3}*{$\tau$} & \multicolumn{2}{c|}{Balanced} &  \multicolumn{2}{c|}{Unbalanced} \\ 
% 		\cline{3-6}
% 		 && Time (s) & Comm (MB) &  Time (s) & Comm (MB) \\
%          \hline
%          $10^3 $ &  $722$ & $0.8$ & $1.06$  & $0.4$ & $0.95$ \\
%          \hline
%          $10^4 $ &  $954$ & $0.9$ & $4.03$  & $1.1$ & $3.07$ \\
%          \hline
%          $10^5 $ &  $1194$ & $6.0$ & $31.83$  & $6.7$ & $22.17$ \\
%          \hline
%          $10^6 $ &  $1440$ & $49.8$ & $307.6$  & $57.4$ & $210.78$ \\
%          \hline
%          $10^7 $ &  $1690$ & $502.5$ & $3063.02$  & $568.4$ & $2094.88$ \\
%          \hline
% 	\end{tabular}
% \end{table*}

\begin{table}[h]  \footnotesize
	\caption{Performance of DPCA-PSI for balanced input sets with different intersection ratio. Each set contains three ID columns with no payloads. The size of the input sets is $10^6$. The network setting is LAN with $10$Gb bandwidth and $0.2$ms latency.}  
 	\centering\setlength{\extrarowheight}{2pt}
	\label{tbl:benchmark_intersection_ratio}

	\begin{tabular} {c|r|r}%{|p{2cm}|p{2cm}|p{2cm}|}
		\toprule
		Intersection ratio & Time (sec) & Comm. (MB) \\ 
            \hline
            $10\%$ & $59.2$ & $369.4$ \\
            \hline
            $30\%$ & $54.8$ & $338.5$ \\
            \hline
            $50\%$ & $49.8$ & $307.6$ \\
            \hline
            $70\%$ & $45.4$ & $276.7$ \\
            \hline
            $90\%$ & $40.6$ & $245.8$ \\
         \bottomrule
	\end{tabular}
\end{table}

\subsection{Comparison with Circuit-PSI}
We also compare the performance 
with circuit-PSI with details shown in Appendix~\ref{app:circuit-psi}.

% Adapting circuit-PSI protocols to support multi-ID matching is a significant challenge, especially with waterfall matching logic. Therefore, we only compare the performance with~\cite{popets/ChandranGS22} in the single-ID setting. 
% We obtain their C++ implementation from GitHub and test their performance with the same hardware settings. 
% Since our focus is on evaluating the performance of the PSI component, payloads are not included in this experiment. 
% The benchmark results are presented in Table~\ref{tbl:benchmark_circuit_psi}. We observe that the main advantage of DPCA-PSI is the communication cost, which is around $10\times$ cheaper than Circuit-PSI. Consequently, DPCA-PSI performs much better than PSM2~\cite{popets/ChandranGS22}, especially in slower network settings. 
% % Furthermore, when considering payloads, DPCA-PSI will demonstrate a more obvious advantage. This is because the input size of the downstream MPC in DPCA-PSI is determined by the intersection set size, which can be significantly smaller than that of circuit-PSI (the size of both parties' input sets).

% \begin{table*}[!htbp]  \footnotesize
% 	\centering\setlength{\extrarowheight}{2pt}
% 	\caption{Performance comparison between DPCA-PSI and Circuit PSI~\cite{popets/ChandranGS22}. Each party has one column as the ID and no payloads. (PSM2 is the protocol presented in \cite{popets/ChandranGS22})}  
% 	\label{tbl:benchmark_circuit_psi}

% 	\begin{tabular} {c|r|r|r|r|r|r|r|r} %{|p{1.2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
% 		\toprule
% 		\multirow{3}*{Input size} & \multicolumn{6}{c|}{Time (sec)} &  \multicolumn{2}{c}{Comm. (MB)} \\ 
% 		\cline{2-7}
%           & \multicolumn{2}{c|}{$10$Gb \& $0.2$ms} & \multicolumn{2}{c|}{$100$Mb \& $50$ms}& \multicolumn{2}{c|}{$10$Mb \& $50$ms} & \multicolumn{2}{c}{}\\
% 		\cline{2-9}
% 		 & PSM2 & DPCA-PSI & PSM2 & DPCA-PSI &PSM2 & DPCA-PSI &PSM2 & DPCA-PSI \\
%          \hline
%          $10^3 $ & $0.85$ & $0.71$ & $5.82$ & $2.66$ & $7.15$ & $4.27$ & $3.57$ & $0.11$ \\
%          \hline
%          $10^4 $ & $1.02$ & $1.07$ & $7.81$ & $3.47$ & $12.46$ & $4.72$ & $12.04$ & $0.89$ \\
%          \hline
%          $10^5 $ & $2.70$ & $2.33$ & $17.04$ & $6.10$ & $75.03$ & $12.42$ & $102.37$ & $8.62$ \\
%          \hline
%          $10^6 $ & $22.71 $ & $16.09$ & $89.78$ & $27.76$ & $672.75$ & $95.95$ & $1075.56$ & $85.57$ \\
%          \hline
%          $10^7 $ & $230.06$ & $163.28$ & $806.39$ & $241.95$ & $6305.37$ & $934.67$ & $10756.52$ & $858.36$ \\
%          \bottomrule
% 	\end{tabular}
% \end{table*}


% \subsection{Trade-off between Performance and Privacy}

% Note that if we require the protocol to be secure against multiple PSI queries, more dummy elements have to be added. Consequently, the performance of DPCA-PSI decreases due to the increasing input sets. We conduct experiments to illustrate this influence. In these experiments, we fix all the parameters except the DP parameters $\epsilon$ and $T$. The experiment results are available in Table~\ref{tbl:benchmark_dp}. We observe that with small input sets (e.g., $10^4$), the performance decreases as the DP parameters become stricter. However, for large input sets, the performance almost remains the same. It is because the dummy set size is too small to influence the overall performance even with the most strict DP parameters. Therefore, we can benefit from better privacy protection with almost no cost when the input set is large.

% \begin{table}[!htbp]  \footnotesize
% 	\caption{Execution time (seconds) of DPCA-PSI with different differential privacy parameters. Each set contains three columns of IDs with one column of payloads. The network setting is LAN with $10$Gb bandwidth and $0.2$ms latency. $n$ represents the size of input sets.}  
%  	\centering\setlength{\extrarowheight}{2pt}
% 	\label{tbl:benchmark_dp}

% 	\begin{tabular} {p{0.4cm}|p{0.8cm}|p{0.95cm}|p{0.95cm}|p{0.8cm}|p{0.95cm}|p{0.95cm}}%{c|r|r|r|r|r|r}
% 		\toprule
% 		\multirow{3}*{N}  & \multicolumn{3}{c|}{$\epsilon = 2$} &  \multicolumn{3}{c}{$\epsilon = 4$} \\ 
% 		\cline{2-7}
% 		       & $T = 6$ & $T = 10$ &  $T = 20$ & $T = 6$ & $T = 10$ &  $T = 20$ \\
%          \hline
%          $10^4 $ &  $3.0$ & $3.3$ & $3.6$  & $2.4$ & $2.6$ & $3.0$\\
%          \hline
%          $10^5 $ &  $18.4$ & $18.5$ & $19.7$  & $18.3$ & $18.4$ & $18.5$\\
%          \bottomrule

% 	\end{tabular}
% \end{table}


